High-Level Synthesis for Packet-Processing Pipelines

Compiling high-level programs to target high-speed packet-processing pipelines is a challenging combinatorial optimization problem. The compiler must configure the pipeline's resources to match the high-level semantics of the program, while packing all of the program's computation into the pipeline's limited resources. State of the art approaches tackle individual aspects of this problem. Yet, they miss opportunities to efficiently produce globally high-quality outcomes. We argue that High-Level Synthesis (HLS), previously applied to ASIC/FPGA design, is the right framework to decompose the compilation problem for pipelines into smaller pieces with modular solutions. We design an HLS-based compiler that works in three phases. Transformation rewrites programs to use more abundant pipeline resources, avoiding scarce ones. Synthesis breaks complex transactional code into configurations of pipelined compute units. Allocation maps the program's compute and memory to the hardware resources. We prototype these ideas in a compiler, CaT, which targets the Tofino pipeline and a cycle-accurate simulator of a Verilog hardware model of an RMT pipeline. CaT can handle programs that existing compilers cannot currently run on pipelines, generating code faster than existing compilers, while using fewer pipeline resources.

==> acks.tex <==
% Kexin Jin

==> background.tex <==
\section{Motivation}
\label{sec:background}
% \aarti{please add references} 

As motivation for our work, we first overview language constructs supported by the P4 programming language, but not yet supported by existing compilers. Second, we show several examples that illustrate weaknesses in resource allocation of existing compilers, e.g., the compiler for the Tofino programmable switch~\cite{tofino}.

\subsection{Programming language and compilers}
With the popularity of programmable network substrates, several languages have emerged to support packet processing, e.g. P4-14, P4-16~\cite{p4_16}, SNAP~\cite{snap}, Marple~\cite{marple}, and Domino~\cite{domino}, Lyra~\cite{lyra}, $\mu$P4~\cite{microp4}. In order to simplify programming, transactional constructs for packet processing 
are supported in some of these languages such as P4-16~\cite{p4_16} and Domino~\cite{domino}. However, currently no existing commercial compiler can handle such transactional constructs. For example, the Tofino compiler rejects P4-16~\cite{p4_16} programs with atomic constructs.
% For example, if a P4-16~\cite{p4_16} program with atomic constructs is fed into the Tofino compiler, it is rejected immediately because the compiler cannot support atomic constructs. 
In addition, if there are sequential dependencies within a \emph{non-atomic} action block (e.g., pkt.x = pkt.y + pkt.z followed by pkt.c = pkt.x + 1), the Tofino compiler rejects the program despite it being valid P4 code. This is because multiple ALUs are required in consecutive stages to express the computation of a single action block. However, the Tofino compiler currently lacks the ability to perform code generation to split a single action block into multiple fragments and map each fragment to a separate ALU. This lack of transaction support in compilers presents a problem for programmers who wish to write packet-processing code with transactional semantics. They have to manually generate code \xiangyu{and allocate the generated code to corresponding stages} for the target architectures, which is an error-prone and time-consuming process.
% For example, if a P4-16~\cite{p4_16} program with atomic constructs is fed into the Tofino compiler, the compiler rejects the program immediately because it can not support the atomic construct. In addition to not supporting such atomic action blocks, even for non-atomic actions, if the programmer adds some sequential dependencies within one action block (e.g., pkt.x = pkt.y + pkt.z followed by pkt.c = pkt.x + 1), the Tofino compiler will also reject the program despite it being valid P4. This is because multiple ALUs are required in consecutive stages to express the computation of a single action block. However, the Tofino compiler currently lacks the ability to perform code generation to split the single action block into multiple fragments and map each fragment to a separate ALU. This lack of transaction support in compilers presents a problem for programmers who wish to write packet-processing code with transactional semantics. They have to manually generate code for the target architectures, making the whole process error-prone and time-consuming. 

%. \aarti{Is the term sequential dependency well-known here? Is any sequential dependency rejected, or some kinds?} \xg{All sequential dependency rejected as far as the computation of one particular variable cannot be finished within one ALU. But I am not sure whether this statement is clear or not to the reader}
%This brings a problem for programmers who are trying to write packet processing code. On the one hand, they have strong willingness to write a program which preserves transactional semantics by using atomic constructs or add some sequential dependencies within an action block; on the other hand, the lack of ability from the existing compiler makes the compilation process of these written programs impossible, forcing companies to hire experienced engineers who are familiar with both programming language and target architecture so as to manually generate code for these architectures to preserve transactional semantics. This whole process then becomes unnecessarily error-prone and time-consuming. 
% This brings a problem for program writers
% Engineers who are familiar with both language and architecture are needed to . Error-prone and time-consuming

\subsection{Resource allocation in existing compilers}

\begin{figure}[t!]
    \centering
    % \vspace{-0.2in}
    \includegraphics[width = \columnwidth]{figures/very_important_ex.pdf}
    \vspace{-0.2in}
    \begin{tiny}
    % \caption{Two syntactically different versions of the same P4 program.}
    \caption{Two versions of the same P4 program.}
    %semantically equivalent versions of a P4 program. The compiled Version 1 uses more resource than compiled Version 2.}
    \label{fig:motivating_example}
    \end{tiny}
    % \myvspace{-0.15in}
\end{figure}

\begin{figure}[t!]
    \centering
    \vspace{-0.2in}
    \includegraphics[width = \columnwidth]{figures/Dependency_graph.pdf}
    \vspace{-0.25in}
    \begin{tiny}
    \caption{Dependency graph for versions 1 and 2.}
    \label{fig:dependency_dag}
    \end{tiny}
    % \myvspace{-0.15in}
\end{figure}

\begin{figure}[t!]
    \centering
    \vspace{-0.18in}
    \includegraphics[width = \columnwidth,scale=3.0]{figures/Resource_sche.pdf}
    \vspace{-0.2in}
    \begin{tiny}
    % \caption{Resource allocation results from the Tofino compiler for version 1 and version 2.}
     \caption{Tofino resource usage for versions 1 and 2.}
    \label{fig:resource_allo}
    \end{tiny}
    \vspace{-0.13in}
\end{figure}

% \begin{figure}[t!]
%     \centering
%     \vspace{-0.1in}
%     \includegraphics[width = \columnwidth,scale=3.0]{hotnets21-template/Figures/Resource_alloc1.pdf}
%     \vspace{-0.25in}
%     \begin{tiny}
%     \caption{Resource allocation from the Tofino compiler for version 1.}
%     \label{fig:version1_resource}
%     \end{tiny}
%     \vspace{-0.13in}
% \end{figure}

% \begin{figure}[t!]
%     \centering
%     \includegraphics[width = \columnwidth,scale=3.0]{hotnets21-template/Figures/Resource_alloc2.pdf}
%     \vspace{-0.25in}
%     \begin{tiny}
%     \caption{Resource allocation from the Tofino compiler for version 2. }
%     \label{fig:version2_resource}
%     \end{tiny}
%     \vspace{-0.06in}
% \end{figure}

\begin{figure}[t!]
    \centering
    % \vspace{-0.1in}
    \vspace{-0.28in}
    \includegraphics[width = \columnwidth,scale=3.0]{figures/Dependency_graph1.pdf}
    \vspace{-0.25in}
    \begin{tiny}
    \caption{Dependency graph for simplified benchmark No.2.}
    %when we assume Tofino switch can allow at most six tables per stage.}
    \label{fig:dep_graph_bench2}
    \end{tiny}
    \vspace{-0.1in}
\end{figure}

\begin{figure}[t!]
    \centering
    \vspace{-0.1in}
    \includegraphics[width = \columnwidth,scale=3.0]{figures/Dependency_graph2.pdf}
    \vspace{-0.25in}
    \begin{tiny}
    \caption{Dependency graph for simplified benchmark No.3}
    %when we assume Tofino switch can allow at most two tables per stage}
    \label{fig:dep_graph_bench3}
    \end{tiny}
    \vspace{-0.23in}
\end{figure}
Even for programs without any atomic constructs \xiangyu{and without any sequential dependency within all action blocks}, code produced by the some commercial compiler such as Tofino compiler can often use more resources than strictly needed.
We conducted some simple experiments with the Tofino compiler and found that the final resource allocation depends on the \emph{syntax} of the input program, even for two programs that are semantically equivalent. For example, given the same semantics (i.e., read-write dependencies between tables), the sequence of tables that a programmer writes in a control block within a P4 program can affect the final number of stages needed by the Tofino compiler.
%As a simplified example, consider two
Two such simplified versions with different sequences are shown in Figure~\ref{fig:motivating_example}, where both versions generate the same dependency graph shown in Figure~\ref{fig:dependency_dag}.
%as they are semantically equivalent. 
Tofino limits the number of tables that can be placed within a single stage of the pipeline. For ease of exposition, we assume that the limit is at most two tables per pipeline stage.\footnote{The actual Tofino limit is somewhat higher, but we have observed this problem with real programs similar to Figure~\ref{fig:dependency_dag} fed to the Tofino compiler as well.} For the code produced by the Tofino compiler, the P4 program in version 1 needs four stages, while the P4 program in version 2 needs only three stages, shown in Figure~\ref{fig:resource_allo}. In other words, two different versions that write the same functionality might lead to differences in resource usage. 

It is not hard to find similar issues with other examples in Table~\ref{table:Resource usage comparison}. In general, we found these issues when the dependency graph is somewhat complex, e.g., with intricate dependency relationships between tables and long dependency paths, similar to Figure~\ref{fig:dep_graph_bench2} and Figure~\ref{fig:dep_graph_bench3} or some tables have complex action with multiple match fields, both of which makes it harder for Tofino compiler to analyze the dependency relationship and allocate corresponding resources properly. Due to space limitations, the benchmark examples shown in the figures are simplified;
%version of real examples, but 
we report on the actual number of stages used by real benchmark programs compiled to Tofino in our experiments (\S\ref{sec:eval}).
%\aarti{to save space, we could put stages of v1 and v2 in a single figure, instead of fig 3 and 4.} \ngs{Agree with Aarti. I also suggest moving benchmark2 and benchmark3 to the appendix since we don't discuss it in the main body of the text.} %\aarti{appendices are not allowed, I think. Maybe we can make the P4 benchmarks available anonymously so people can check it with Tofino compiler?}

%it is possible that the actually required resource can be fit into the target architecture while the sub-optimal allocation wants more than what is available, making the compiler 
%stages are relatively sufficient and Tofino compiler successfully compiles a program using more stages than needed, it 
To make things worse, compiling programs to pipeline architectures is all-or-nothing. 
%which means that a successfully compiled program can run at the pipeline's line rate, but a program rejected by the compiler cannot run at all. 
Therefore, if the compiler mistakenly decides that a program requires more resources than what the pipeline provides, 
%even though what the program strictly needs is within the pipeline's resource availability, 
the compiler may \emph{incorrectly} reject the program.\xiangyu{Is it better to show examples illustrating reject and accept difference?} Even when compilation succeeds, a sub-optimal resource allocation may lead to larger packet-processing latency due to an increase in the number of pipeline stages. This increase in latency \xiangyu{and power consumption?} can be significant in application areas such as high frequency trading~\cite{high_freq_trade}.
%because each pipeline stage can add 10s of ns of additional latency.

%\ngs{It wasn't obvious to me that (i) HFT uses general switch pipelines, (ii) programs with fewer stages actually reduce total latency. Adding citations will help. }

%\aarti{could we add a reference and/or quantify this -- each additional pipeline stage costs roughly 20-30 nanosec?}

% \subsection{Leverage ILP for resource allocation}
% We use the ILP solver to do resource allocation (e.g. ALUs, logical table IDs) for the given packet-processing program to target architecture while minimizing the total number of stages. Because both the constraints and objective function are integer-valued, it is reasonable to consider Integer Linear Programming (ILP). In general, an integer linear programming problem is a mathematical optimization program in which all of the variables are restricted to be integers. In our resource allocation process, if we can represent all constraints, including resource constraints and dependency constraints, and objective function as a linear combination of variables, then we can leverage fast ILP solvers (e.g. Gurobi) to generate the allocation results.
\subsection{Motivating more powerful compilers}
The purpose of building a new compiler is to tackle the issue of the lack of code generation functionality and bad resource allocation behavior. 
Compiler is a bridge between program writer and underlying hardware
Compiler designer are usually more familiar with the target hardware
Also provide programmers with the freedom to update the compiler by parameterizing the resource constraints.
Can fully utilize the hardware resources without wasting any of them
Our goal is to extend the 


==> background_asplos23.tex <==
\section{Background and Overview}
% QUESTION: What is the goal/contribution of the work in one sentence?
\subsection{Packet-processing pipelines}
The compiler target for this paper is a programmable packet-processing pipeline following the Reconfigurable Match-Action Tables (RMT) architecture~\cite{rmt}. 
Such pipelines are present in commercially available programmable switches such as the Barefoot Tofino~\cite{tofino}, Broadcom Trident, and Mellanox Spectrum, and NICs such as the Pensando DPU.  An RMT-style pipeline consists of (i) a programmable packet parser, (ii) a number of stages
each of which is structured around the paradigm of \emph{match-action processing}: specific headers from incoming packets are looked up in a table (match) and if the match succeeds, the packet is modified 
% \xiangyu{we should use "transformed" or "modified" or "updated"?} 
in some way (action).

The match can involve exactly matching the header bits to entries in the table or 
% \xiangyu{or --> and}
allow wildcard/don't-care bits within the table entries. The action modifies multiple packet headers using a very long instruction word (VLIW) architecture: different headers within the packet can be independently modified by controlling the appropriate opcode within the VLIW instruction. Actions can also atomically modify pipeline state in addition to packet headers such that the updated state is visible to the next packet.

To support line-rate packet processing on all ports even for small packet sizes, such pipelines constrain their match and action units. Only a certain number of bits from the packet can be extracted to form the match key for the lookup tables and there are a limited number of lookup tables in each stage. Actions are also
%\xiangyu{maybe we should remove "similarly" since ALU is actually not similar to other types of resources} 
constrained so that a stateful update must complete within a clock cycle before the next packet arrives.

The job of the compiler then becomes 
%one of\xiangyu{maybe remove "one of"} 
solving a constrained optimization problem where a program's computations must be mapped to the constraints of the pipeline. But, in exchange for these constraints, performance\xiangyu{Not sure what does performance here mean? the compilation time or the quality of compiled program?} of packet-processing programs can typically be predicted at compile time.\footnote{An exception to this is when packets are recirculated into the pipeline for a second or subsequent pass---a more rarely used feature.}
% .\doris{an extra dot?} 
These features\doris{Do these features refer to both the constraints and performance?} make such pipelines (and their compilers) more similar to spatial substrates such as FPGAs and CGRAs, rather than a program-counter-based architecture such as a CPU or GPU.

\subsection{Related work}
\label{sec:prior-compilers}
%\Para{New DSLs\xiangyu{Since this is the first time DSL shows up, should we give the full name Domain-specific languages as well?}.}
\para{New domain specific languages (DSLs)}
Several new DSLs have been proposed to program these emerging packet pipelines. The most widely used examples are P4 and NPL, both of which share many similarities. Several academic projects have proposed new DSLs or extensions to P4 to remedy many of its shortcomings. For instance, microP4~\cite{microp4} adds modularity to P4. Lyra~\cite{lyra} addresses the issue of portability of programs across multiple devices. Lyra and Flighplan~\cite{flightplan} address the problem of partitioning a program automatically across multiple devices. Lucid~\cite{lucid} introduces an event-driven programming model for control applications in the data plane. P4All~\cite{p4all} extends P4 by supporting elastic data structures, whose size can grow and shrink dynamically based on the availability of switch resources. Domino~\cite{domino} is a DSL that supports transactional packet processing: a programmer specifies a block of code that is executed on each packet in isolation from other packets.

%\Para{Rewrite rules.\xiangyu{Call it program rewrite?}}
\para{Program rewrite rules}
The open-source reference P4 compiler~\cite{p4c}, which is the foundation for most P4 compilers including the widely used Tofino compiler~\cite{p4sde}, employs rewrite rules to turn the input P4 program into successively simpler P4 programs. These rewrite rules consist of classical optimizations like common subexpression elimination and constant folding. Rewrite rules are also employed by Cetus~\cite{cetus} to merge tables in different stages into a single ``cartesian-product'' table in a single stage, thereby saving on the number of stages---a very scarce resource on packet-processing pipelines. Such rewrite rules are also employed in the compilers of new DSLs such as Lucid~\cite{lucid} and Lyra~\cite{lyra}.

% TODO: ALUs vs. action units: be clear about the distinction.
%\Para{Code generation.}
\para{Code generation}
Domino~\cite{domino} and Chipmunk~\cite{chipmunk} tackle the problem of code generation (or instruction selection) in programmable packet-processing pipelines. The code generation problem takes a transactional description of packet processing and breaks it down into smaller chunks that can each be executed within one pipeline stage, respecting the limited capabilities of each stage's VLIW ALUs. The code generation problem is similar to the problem of instruction selection in a classical compiler with the stateful and stateless action units defining the instruction set that the compiler is targeting. Domino uses largely rewrite rules and a small amount of 
% \xiangyu{Is it a little bit subjective to call this "a small amount"} 
program synthesis for code generation, while Chipmunk employs exhaustive search via program synthesis, resulting in a better likelihood of actually compiling feasible transactions into a pipeline's resources.

%\Para{Resource allocation.}
\para{Resource allocation}
Several projects tackle the problem of allocating a program's computation and data structures to the finite resources of a pipeline, e.g., mapping actions to action units and tables to memory blocks. This allocation problem can be posed as an ILP~\cite{lavanya_nsdi15, p4all} or an SMT problem~\cite{lyra}, after which the appropriate solver engine can be invoked. A key requirement for this approach is exact or imperfect knowledge of the underlying hardware target's resources and their constraints. Hence, the efficiency of such resource allocation depends on how precisely the constraints of the hardware are modeled. If implemented with a precise model of the hardware, ILP-based techniques can improve resource allocation relative to greedy heuristics for resource allocation.
% ~\cite{lavanya_nsdi15} (also see Figure~\ref{fig:ilp})\xiangyu{since this figure was in the paper, should we put this figure into appendix?}.

\begin{table*}[]
    \centering
    \begin{scriptsize}
    \begin{tabular}{|c|c|c|c|c|c|}
         \hline
         Project & Resource Allocation & Code generation & Rewrite rules & Portability & Language constructs \\
         \hline
         Domino~\cite{domino} & \xmark & Rewriting, program synthesis & Yes & Atom templates & Packet transactions \\
         \hline 
         Chipmunk~\cite{chipmunk} & \xmark & Program synthesis & \xmark &  ALU DSL & Packet transactions\\
         \hline
         Lyra~\cite{lyra} & SMT & \xmark & Yes & SMT constraints & Network-wide programs \\
         \hline
         Flightplan~\cite{flightplan} & Resource rules & Resource rules & \xmark & Yes & Network-wide programs \\
         \hline
         Cetus~\cite{cetus} & Table Merging + PHV Sharing & \xmark & Yes & Same as P4 & \xmark \\
         \hline
         P4All~\cite{p4all} & ILP & \xmark & \xmark & \xmark & Elastic data structures \\
         \hline
         Jose et al.~\cite{lavanya_nsdi15} & ILP & \xmark & \xmark & ILP constraints & \xmark \\
         \hline
         Lucid~\cite{lucid} & \xmark & memops & \xmark &  \xmark & Event-driven programming \\
         \hline
         p4c & \xmark & \xmark & Yes & Target architecture description & \xmark \\
         \hline
         \sysname & ILP/SMT & Min-depth tree algorithm & Yes & ILP constraints, ALU grammar & P4's atomic construct \\
         \hline
    \end{tabular}
    \caption{\sysname unifies prior work on code generation, resource allocation, and code optimization, and does so within the context of the P4 language, without needing a new DSL.
    \ruijie{Could we potentially add coloring to this table for readability? }}
    \xiangyu{Make table heading bold in all tables}
    % The rewrite rules column also has some inconsistent naming conventions?
    \end{scriptsize}
    \label{tab:priorWorks}
\end{table*}

%TODO: Figure of the overall workflow for our compiler.
\subsection{Our approach: HLS for packet pipelines}
\sysname is an end-to-end compiler for P4-16 programs that takes inspiration from HLS to provide both: (1) a high-level of abstraction for specifying packet-processing functionality, and (2) high quality of the compiler-produced implementation. While prior approaches to HLS for ASICs and FPGAs have sometimes caused poor quality of result of the implementation, we believe that the narrower domain of packet-processing pipelines gives us an ability to apply HLS more gainfully than has been done before.

\begin{figure}[t]
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.39\textwidth]{figures/siphash.pdf}
    \vspace*{-0.1in}
    \caption{Motivating Example ME-1: Siphash pseudo-code was manually split into four stages and rewritten to P4 by others~\cite{siphash}.}
%    \vspace*{-0.2in}
    \label{fig:motivation_siphash}
    \vspace*{-0.1in}
\end{figure}

To raise the level of abstraction, we leverage P4's atomic annotation, based on the concept of packet transactions from Domino~\cite{domino}. The atomic annotation allows a programmer to mark a block of packet-processing code for transactional execution: all statements within the block will either be executed or not, without any appearance of interleaving of the same block executed for other packets. We start with this higher level of abstraction because it is a convenient way to express algorithmic portions of packet processing, especially those involving state, as demonstrated in several previous projects~\cite{domino, marple, pifo, mp5}. 

To illustrate the weaknesses of current compilers,
%benefits of compiler support for high-level transactions, 
consider a motivating example (ME-1) shown in Figure~\ref{fig:motivation_siphash} that shows pseudo-code for the SipHash algorithm~\cite{siphash}. The authors initially started with a high-level description
% transactional description
% \xiangyu{Since there is no stateful vars in siphash, should we still mention transactional?}\aarti{say high-level?} 
of the algorithm (~\cite{siphash}[Table 3]). They then manually changed it into a pipelined implementation (~\cite{siphash}[Table 4])\xiangyu{check table number}; a good compiler \emph{should} automate this. \emph{CaT can successfully handle this example (discussed in \S\ref{ssec:comparison}), without requiring a user to make manual changes.}
%\ruijie{Two questions: 1, where is table 3? let's use a latex command to crossref it. 2, should we present a figure of pseudocode illustrating a single SipHash round?}
% \xiangyu{I think table3 means table3 in siphash paper. But I agree, maybe we should say Table 3 in ~\cite{siphash}. As for the psedocode of siphash, I am not sure whether we still have space to present or not. Maybe pointing to one part of the paper or cite the corresponding github link as an alternative?}
%\aarti{I too think we should present a small figure showing the relevant pseduo-code of siphash, which should highlight that it is transactional code that requires multiple stages -- which would otherwise require manual changes to compile. }

\begin{figure}[!t]
    \centering
    % \vspace{-0.2in}
    \includegraphics[width = 
    \columnwidth]{figures/ret_workflow.pdf}
    % \vspace{-0.3in}
    \vspace{-0.2in}
    \begin{tiny}
    \caption{The workflow of CaT compiler.}
    %\as{Can we remove Tofino compiler from this picture?}}
    \label{fig:hls_workflow}
    \end{tiny}
    \vspace{-0.25in}
    % \myvspace{-0.15in}
\end{figure}

To produce high quality implementations, \sysname combines ideas from several prior projects (Table~\ref{tab:priorWorks}) into an end-to-end system for the first time. We use an HLS workflow to divide up the process of compiling a P4-16 program into three phases, as shown in Figure~\ref{fig:hls_workflow}. 
First, \emph{resource transformations} rewrite packet-processing programs in P4 from one form (that makes use of a scarce resource) to another form (that makes use of a more abundant resource). Second, \emph{resource synthesis} employs a novel algorithm based on a program synthesis engine to synthesize 
%low-level configurations 
resource graphs with hardware ALUs, from a high-level transactional specification of a match-action table's action functionality. Third, \emph{resource allocation} employs ILP or %\xiangyu{and -> or} 
SMT solvers to allocate computations and data structures to memory blocks and action units, while respecting program dependencies and per-stage resource constraints.
Notably, our HLS workflow works within the confines of the widely used P4 ecosystem without requiring the development of a new DSL for packet processing.

\begin{table*}[!ht]
\scriptsize
\begin{tabular}{|p{3cm}|p{3cm}|p{3cm}|p{3.75cm}|p{3.25cm}|p{3cm}|}\hline
CaT compiler phase & Technique & Builds on prior work & Differences in CaT & Other complementary work \\\hline
1: Resource transformation (corresponds to HLS code transformation) & Rewrite rules & LLVM~\cite{llvm}, HLS~\cite{hls, hls_fpga}, p4c~\cite{p4c} & Rewrite rules target RMT, based on novel guarded dependency analysis & p4c~\cite{p4c} performs platform-independent rewrites, Cetus~\cite{cetus} splits tables  \\ \hline
\multirow{4}{3cm}{2: Resource synthesis (corresponds to HLS operation binding and HLS module selection)} & Preprocessing: branch removal, SSA, SCC for stateful updates & Domino~\cite{domino}, SSA~\cite{ssa}, VLIW~\cite{lam} & no backward control flow (like Domino) & \\ \cline{2-5}
& Simplifications: constant propagation, expression simplification, deadcode elimination & LLVM~\cite{llvm}, HLS code transformation~\cite{hls,hls_fpga} & no backward control flow & \\ \cline{2-5}
& Uses program synthesis for mapping operations to functional units & Chipmunk~\cite{chipmunk} & Novel synthesis procedure: faster and more scalable than Chipmunk, separates queries for stateful and stateless operations & Lucid uses syntactic rules to ensure operations can map to Tofino ALUs \\ \cline{2-5}
& Target portability via parameterizable grammars for functional units & Sketch~\cite{sketch}, Chipmunk~\cite{chipmunk} & synthesizes resource graph (used in Phase 3), not low-level ALU configurations & \\ \hline
\multirow{4}{3cm}{3: Resource allocation (corresponds to HLS scheduling)} & Constraints for match memories & Jose et al.~\cite{lavanya_nsdi15}, Lyra~\cite{lyra} & & \\ \cline{2-5}
& Constraints for multi-stage actions & Domino~\cite{domino}, Chipmunk~\cite{chipmunk} & Uses result of Phase 2 for intra-action dependencies and ALU output propagation & \\ \cline{2-5}
& Constraints for multiple transactions & Domino~\cite{domino}, Chipmunk~\cite{chipmunk} handle a single transaction only & Uses result of Phase 2 for global optimization & \\ \cline{2-5}
& Modeling real hardware constraints (match crossbar, logical tables) in backend FPGA target & Menshen provides a FPGA backend target~\cite{menshen} & & Tofino compiler uses heuristics for resource allocation \\ \hline
\end{tabular}
\caption{CaT in relation to HLS and other related work}\label{tab:hls}
\end{table*}

\subsection{Summary of Contributions}
Our main contribution is an HLS workflow for packet processing pipelines that unifies rewrite rules, code generation, and resource allocation for the first time.
% , and \xiangyu{should we say in the reverse order rewrite rules, code generation, and resource allocation} 
% in the form of our resource allocation, resource synthesis, and resource transformation phases \xiangyu{also reorder here}respectively. 
An additional contribution is our ability to work within the P4 ecosystem without a new DSL. Our key insight is that HLS provides a framework %technique
to decompose the hard combinatorial optimization problem at the heart of RMT compilers into 3 separate and more manageable subproblems. These phases are highlighted in Table~\ref{tab:hls}, 
where the first phase (Resource transformation) corresponds roughly to the code transformation step in HLS, 
the second phase (Resource synthesis) corresponds to operation binding~\cite{hls_asic} or module selection~\cite{hls_fpga} in HLS, and the third phase (Resource allocation) corresponds to the scheduling step in HLS. 
Each of these phases builds on top of well-known prior techniques shown in the table, but with significant differences and novelties in our work (highlighted below, described in detail later). The last column in the table lists prior work with complementary techniques that could potentially be combined in our compiler. 

Beyond unifying these 3 compiler techniques into a single HLS workflow, we also make individual contributions in the three phases, briefly highlighted below.
%code generation, resource allocation, and rewrite rules,\doris{then maybe also reorder here?} highlighted below (and summarized in Table~\ref{tab:hls}.
\begin{CompactEnumerate}
\item Our rewrite engine for resource transformations employs a novel \emph{guarded} dependence analysis, which is more precise than traditional dependency analysis and 
%based on the path condition associated with each P4 statement, which we call \emph{guarded dependency analysis}. 
allows us to exploit more opportunities for parallelism.
%\xiangyu{Since we call it rewrite phase, in addition to mentioning precise dependency analysis, should we also say rewriting the program into a new version which use tables to represent ITE statement?}
\item Our novel algorithm for resource synthesis is
%the min-depth-tree algorithm, is an algorithm 
inspired by circuit synthesis, and uses a program synthesis engine as a subroutine. It separates out stateful updates from stateless updates to decompose the problem 
%from Chipmunk~\cite{chipmunk} 
into smaller and more tractable subproblems than Chipmunk~\cite{chipmunk}, which leads to a significant reduction in runtime, despite needing fewer compute resources. 
Keeping synthesis times low is particularly important for \sysname because the synthesis procedure is run multiple times as a subroutine. 
%within the overall \sysname compiler. 
At the same time, \sysname's synthesizer produces significantly better quality code than Domino~\cite{domino}, and code comparable to that produced by Chipmunk's more expensive synthesizer.
\item Our resource allocation formulation 
%builds on the top of 
is similar to the formulation of Jose et al.~\cite{lavanya_nsdi15} and Lyra~\cite{lyra} for memory blocks, but models other hardware resources in significantly more detail. 
For instance, we model allocation of and constraints on the ALU units in action blocks (which can be determined only after resource synthesis). We also model the number of bits that can be looked up in a match-action table within a single stage. By contrast, Jose et al. work with an abstract model of hardware that wasn't yet built at the time and Lyra tries to optimize a more abstract form of resources (e.g., P4 registers, P4 tables) rather than actual hardware constraints.
\item We built a backend that applies this HLS workflow to the Tofino hardware target and a cycle-accurate simulator of an open-source RMT pipeline from the Menshen project~\cite{menshen}. 
\end{CompactEnumerate}
We present detailed evaluation results for CaT on several benchmark examples (\S\ref{sec:eval}), and show that it can successfully handle motivating examples from real P4 applications without requiring a user to manually make changes.

\subsection{Limitations}
\sysname has two significant limitations. First, it does not deal with the problem of partitioning a \emph{network-wide} program into per-device programs like Flightplan and Lyra do. Instead, our goal is to build a high quality compiler that inputs a P4 program for a \emph{single device} and outputs a high-quality implementation for that device. Second, our backend for Tofino is limited because we lack full knowledge of Tofino's hardware architecture. We believe that our overall ideas still apply to building a full backend for the Tofino chip, but that considerable additional engineering effort will also be needed.\xiangyu{Maybe say additional engineering effort + NDA agreement? Because additional engineering efforts are within our scope but NDA is even without our scope. We have already done whatever we can at this moment}

==> design-old.tex <==
\section{Compiler Design}
\label{sec:design}
Our main approach is centered around decomposing the overall compilation problem into: (1) code generation: to map each action-computation in the program to hardware resources based on its functionality, and (2) resource allocation: to pack resources for all computations and all data structures in all tables to available hardware resources based on resource constraints. Unlike existing compilers, we allow actions where computations may need ALUs in more than one stage---this is needed for allowing rich actions that employ atomic transactions~\cite{domino} and actions that have dependencies between their constituent statements. Effectively, our compiler explores the space of semantically-equivalent program transformations for actions during code generation. 

\subsection{HLS-Inspired Modular Decomposition}
\label{ssec:hls}
The modular decomposition in our compiler approach is inspired by the success of HLS techniques in development of software-hardware systems in modern Systems-on-Chip (SoC) design~\cite{hls}. Starting from a high-level algorithmic description of a hardware component, an HLS tool performs various steps to ultimately generate a lower-level hardware design for an FPGA or ASIC, usually cycle-accurate at the register-transfer level (RTL). These steps include compiling the specification to a (typically) graph-based intermediate representation, \emph{allocating} resources (functional units, storage, buses, etc.), \emph{scheduling} the operations to clock cycles, \emph{binding} the operations to functional units, \emph{binding} the variables to storage elements and transfers to buses, and generating the final clock-accurate RTL design.

In our context, we regard the specification as a P4-16 program and lower it to hardware in the RMT architecture, taking into account the available resources (ALUs, memory, tables, packet header vectors (PHVs), etc.) in pipeline stages. Our code generation procedure can be viewed as finding a schedule for the required operations on the available functional units, while our resource allocation procedure can be viewed as binding the operations/variables/transfers to resources in specific stages of the pipeline. 

Note that we perform code generation \emph{locally}, i.e., for each computation in each table, which keeps the synthesis runtime manageable in practice, even when we use program synthesis to explore the space exhaustively (as shown in \S\ref{sec:eval}). These independent code generation tasks could be parallelized in a future implementation.
%In our current approach, we do not allow these computations to share any resources, e.g., for stateful updates. In future work, we plan to consider static analyses of P4 programs to group together computations that can potentially share resources. Each such group can then form a local unit on which code generation is performed simultaneously. 
On the other hand, we perform resource allocation \emph{globally}, i.e., by considering all computations in all tables in the program. 
%Note that this is enabled by the earlier code generation step, which determines the resources required for each individual computation. When considering packing computations from different tables into the available pipeline stages, our prototype compiler enforces table-level dependencies. This allows computations of independent tables to be potentially packed into the same stage of the hardware pipeline. Our approach can be extended straight-forwardly to pack computations at a finer granularity of operation-level dependencies in future work. 

Our modularization of the compilation problem into local code generation followed by a global resource allocation can be viewed as decomposing the overall problem into smaller subproblems.
%where the local subproblems find solutions to ensure that computations can be mapped to available resources based on functionality, and the global step ensures that all local solutions can be packed into available resources based on capacity. 
This decomposition has the following benefits, in contrast to an alternative approach that would perform code generation and resource allocation \emph{simultaneously} on the full problem. 
\begin{CompactEnumerate}
    \item When performing code generation on small local subproblems, the search space over semantically-equivalent code is smaller, thereby resulting in reasonable performance when using program synthesis (\S\ref{sec:eval}). 
    \item The small subproblems allow us to perform optimization during code generation. In particular, for each subproblem, we find a solution that has a locally minimal depth, i.e., number of pipeline stages. Since the pipeline stages are often a critical resource, the optimized local solutions make it more likely that the global step for packing them based on capacity will succeed. 
    \item It provides the flexibility of looking for a feasible (in addition to an optimal) solution in the global packing step, where the available capacity of hardware resources (e.g., number of pipeline stages) is known. Note that looking for feasible solutions for local subproblems would require guessing suitable hardware capacity limits at the local level, which are not fixed, and too loose or too tight guesses may result in overall compilation failure. Thus, our decomposition enables combining good performance and optimality in local synthesis solutions, with feasible or optimal packing at the global level.
\end{CompactEnumerate}

The general problem of optimal code generation in compilers is known to be NP-complete~\cite{AJU77}, and most compilers decompose the problem in some way to tradeoff optimality for reasonable performance. 
In HLS too, although the tasks to be scheduled are inter-dependent, they are often performed in some sequence to manage the computational complexity of synthesis~\cite{hls}.
%Note that our code generation procedure is applied to one transaction at a time, which keeps the runtime manageable in practice (as shown in \S\ref{sec:eval}). 
%The resource allocation is performed only once for the global P4 program, which allows pipeline stages to be utilized maximally among transactions that are independent. Thus, 

Our approach can be viewed as an \emph{action-level decomposition}, where we perform local code generation for each computation, and then use these results to perform a global resource allocation
for multiple computations. %where multiple computations can be packed within a single stage of the pipelined architecture.
In future work, we plan to perform additional static analyses of P4 programs: to group together computations that can potentially share resources, and to identify operation-level dependencies at a finer level of granularity than table-level dependencies. Each such group can then form a local unit on which code generation is performed, and we can consider operation-level dependencies to further improve packing during resource allocation. 

%This scheme provides an effective transaction-level decomposition of the compilation problem. 
%This transaction-level decomposition is another contribution, providing a crucial first step in building compiler support for transactions.
%For code generation, we provide local optimality guarantees within each transaction (\S\ref{sec:codegne}; for resource allocation, our ILP-based method (\S\ref{sec:ilp}) provides optimality for the target cost. 
%The purpose of code generation is to map each node in $C$ to some hardware resource, e.g., a stateless/stateful ALU, such that the outputs and state updates are implemented correctly. 
%\subsection{High-level overview}
%Our compiler consists of two main phases. In the first phase, we perform \emph{code generation} for each transaction in the P4 program.
%, starting from a \emph{computation graph} $C$ that represents the transaction as a graph of dependencies. 
%The result of our code generation is a \emph{resource graph} $R$, where each node is a hardware resource (e.g., an ALU), and an edge $(u,v)$ denotes that the output of $u$ is connected to the input of $v$. 
%Like the Chipmunk compiler~\cite{chipmunk}, our code generator also leverages automated program synthesis~\cite{sketch,AlurSygus} to exhaustively search over the space of target programs without depending on rewrite rules.
%, but there are significant differences (described later). 
%Given a specification and a grammar, the Sketch tool~\cite{sketch} synthesizes a correct program allowed by the grammar. 
%Our code generation procedure is guaranteed to be correct and we discuss the conditions under which it is optimal.
%in terms of number of pipeline stages.

%available in the hardware pipeline. 
%We identify such independent transactions by analyzing the dependency relations between the tables in the P4 program.
%\todo{add a sentence on the type of table dependencies, and when tables are triggered.} 
%The second phase of our compiler performs \emph{resource allocation} based on integer linear programming (ILP), to allocate resources such as memory blocks and ALUs for P4 language constructs such as tables, expressions, and registers. 
%The constraints for memory blocks are similar to prior work by Jose et al.~\cite{lavanya_nsdi15}. In addition, we consider constraints for other resources, such as ALUs, informed by the resource graphs generated by the code generation phase. 
%The main idea is to allow allocation of resources for \emph{multiple transactions} in each  pipeline stage, as long as the corresponding transactions have no dependencies, which we identify from a table dependency graph similar to that proposed by Jose et al.~\cite{lavanya_nsdi15}.
%Thus, we use the resource graph $R$ of each transaction to enforce {\em intra-table constraints} in the ILP, and use the table dependency graph to enforce {\em inter-table constraints}.
%node resource allocation constraints and input-output connection constraints. The latter kind of constraint enforces that the output of a resource allocated in some stage $i$ is connected as an input to another resource allocated in some stage $j$, where $j > i$, i.e., we do not require $j$ to be $i+1$ necessarily. \emph{This provides flexibility on top of code generation alone, to enable packing the resources for multiple transactions in each pipeline stage.} We can add capacity constraints, such as number of available ALUs per stage, or total number of pipeline stages, and we can optimize with different (linear) objectives, e.g., to minimize the number of pipeline stages or the total number of resources, etc.
%\ani{We could comment out the para below if we are out of space.}
%Aside from novelties in our code generation and resource allocation procedures, we believe that our decomposition of the overall compilation problem into these two phases is also a distinct contribution. 
%The general problem of optimal code generation in compilers is known to be NP-complete~\cite{AJU77}, and most compilers decompose the problem in some way to tradeoff optimality for reasonable performance. Note that our code generation procedure is applied to one transaction at a time, which keeps the runtime manageable in practice (as shown in \S\ref{sec:eval}). (These code generation tasks could be parallelized in a future implementation.) 
%The resource allocation is performed only once for the global P4 program, which allows pipeline stages to be utilized maximally among transactions that are independent. Thus, 
%Effectively, we use the results of \emph{local} per-transaction code generation to perform a \emph{global} transaction-level packing in resource allocation. 
%This scheme provides an effective transaction-level decomposition of the compilation problem. 
%This transaction-level decomposition is another contribution, providing a crucial first step in building compiler support for transactions.
%in packet-processing applications.

%The following subsections describe details of our code generation and resource allocation procedures, along with the compiler workflow that combines them.
% TODO: use one concrete example figure to show how min-depth tree works
\subsection{Code Generation Procedure}
\label{ssec:codegen}
% TODOs: min-depth tree example
We consider each individual action in a program, where action computations are not restricted to a single stage, i.e., we can handle computations that may require multiple stages in the pipeline. In addition, we consider computations with atomic transactional semantics~\cite{domino}, i.e., where stateful updates are required to be performed in a single stage within the pipeline to guarantee atomicity. In the remainder of the paper, we refer to these general action-computations as \emph{transactions}.

For a given transaction, we use a program synthesis tool (SKETCH~\cite{sketch}) to generate \emph{semantically equivalent} code, similar to Chipmunk~\cite{chipmunk}. We note two important differences from Chipmunk.
%of our code generation procedure. 
%for a programmable switch target. 
First, we aim to reduce code generation time by creating \emph{smaller synthesis queries} for SKETCH, rather than invoking it for synthesis of the entire transaction as done in Chipmunk. To mitigate the narrower scope of search in smaller synthesis queries, we perform additional optimizations. Second, %similar to Chipmunk, 
rather than Chipmunk's approach of creating low-level holes in the ALU grid architecture that are filled by SKETCH, 
our code generation procedure is \emph{parameterized by the grammar} that is used by SKETCH in the synthesis queries. 
This enables the same code generation procedure to be used for different hardware backends via grammars. Our compiler currently supports three different grammars: Tofino ALUs~\cite{tofino}, Banzai ALUs~\cite{domino}, and ALUs for our simulation of Menshen~\cite{menshen}; more can be supported as needed without modifying our overall procedure.
%First, the P4 action is converted to an equivalent Domino program which is then transformed using multiple phases, each of which is described below.
The rest of this section describes the steps of our code generation procedure in detail. 

\subsubsection{Preprocessing and Simplification} We use some standard preprocessing steps (e.g., similar to the Domino compiler~\cite{domino}) on the P4 code for a given transaction. In the branch removal step, conditional expressions (if statements) are replaced by conditional assignments to produce straight-line code. Then, temporary packet fields (called read and write flanks) are introduced to store the initial and final values of state variables. The program is then converted to static single-assignment form (SSA)~\cite{ssa} to ensure every variable is written at most once. 
In addition, we perform the following 
% \emph{optimizations}
static analyses during preprocessing: constant folding, expression simplification, and dead code elimination. These static analyses are useful in simplifying the inputs 
%that feed a given function that is the target 
for a SKETCH query. Without these analyses, some functionally-equivalent mutations of our benchmark examples
% require an extremely long time for compilation, 
cannot be compiled, as shown later in our evaluation (\S\ref{ssec:codegen-exp}).  
% Unlike the Domino compiler, we do not convert each statement to three-address code as this can introduce dependencies that increase the number of stages required.

\begin{algorithm}
\DontPrintSemicolon
\SetAlgoLined
\KwIn{Computation graph $G_C = (V, E)$ where $V = V_{stateful} \cup V_{stateless}$.}
\KwOut{Synthesized code for each primary output (PO) and each input to a stateful ALU}
\SetKwFunction{Fmerge}{tryMerge}
\tcp{\scriptsize{Step 1: Check ALUs for stateful updates}}
\For{$v \in V_{stateful}$}
{
success := querySketchStateful(stateVar(v), v)\;
\textbf{assert} success == true\;
    % \If{success == false}{
    %     \Return Error
    % }
}
\tcp{\scriptsize{Step 2: Pack more into stateful ALUs}}
%\For{$v \in V$ in reverse topological order}
%{
%    \For{$u \in pred(v)$}
%    {
%        \If{at least one of $v$, $u$ is stateful and safeToMerge(u, v)}
%        {
%           tryMerge($G_c$, $u$, $v$)\;
%        }
%    }
%}
\For{$(u,v) \in E$, where one of $u$, $v$ is stateful}
    { tryMerge($G_c$, $u$, $v$)\; }
% \For{$v \in V_{stateful}$ in reverse topological order}
% {
%     \For{$u \in pred(v)$}{
%         v = mergeUsingSketch($G_c$, u, v)\;
%     }
% }

\tcp{\scriptsize{Step 3: Synthesize min-depth tree for stateless code}}
O := $POs \cup \{inputs(v) | v \in V_{stateful}\}$\;
\For{$o \in O$}{
%%    \tcp{Find the Backwards Cone of Influence (BCI) of o}
    spec := computeBCI(o) \tcp*{\scriptsize{spec of o}} 
    i := 1 \tcp*{\scriptsize{depth of solution tree}}
    \While{$i \leq $ numPipelinedStages}{
        success := querySketchStateless(o, spec, i)\;
        \If{success == true}{
            \textbf{break} } 
        i++ \tcp*{\scriptsize{increment depth}}
    }
}
%\tcp{Try merging $u$ and $v$ if they fit in a stateful ALU}
%\SetKwProg{Fn}{Function}{:}{}
%\Fn{\Fmerge{$G_c$, $u$, $v$}}{
%    $w$ = union($u$, $v$) \tcp*{combined logic}
%    \If{$\vert inputs(w) \vert$ and $\vert outputs(w) \vert$ meet ALU requirements}{
%        success := querySketchStateful(outputs(w), w)\;
%        \If{success == true}{
%            Replace $u$ and $v$ by $w$ in $G_c$\;
%           Update $V$, $V_{stateful}$, $V_{stateless}$\;
%        }
%    }
%}
\caption{Code Generation Procedure}
\label{alg:1}
\vspace*{-0.1in}
\end{algorithm}

\vspace*{-0.1in}
%\Para{Computation graph construction}
\subsubsection{Computation graph construction}
A dependency graph is constructed from the preprocessed program with nodes for each program statement and an edge for each Read-After-Write (RAW) dependency.\footnote{Conversion to SSA form removes Write-After-Write and Write-After-Read dependencies.} Edges are also added between the read and write flanks of each state variable. The strongly connected components (SCCs) of this graph correspond to stateful updates, which are condensed to form a \emph{computation graph} $G$. Thus, $G$ is a directed acyclic graph (DAG) with nodes for program computations (some with stateful updates) and edges for RAW dependencies.\footnote{This is similar to the DAG generated by the Domino compiler, except that nodes need not be in three-address code.} The sources of $G$ (excluding state variables) are called primary inputs (PIs), 
%i.e., (SSA) variables that are used and not defined, typically 
i.e., input packet fields that are used in the computation. 
%of $C$ are the variables which are used and not defined, i.e., the initial packet field variables.
The sinks of $G$ (excluding state variables) are called primary outputs (POs). 
%i.e., packet field variables with the largest SSA index -- these represent 
%typically 
These correspond to the final values written to packet fields. 
%\ngs{Minor: We don't consider initial state values as PIs (or final state values POs), wondering if we can mention that explicitly somewhere as I was wondering about state after the last sentence.}\aarti{added now}

\subsubsection{Code generation using program synthesis queries}
Given a computation graph $G$, we synthesize code for the POs (packet fields) and state variables such that they are functionally equivalent to the transaction program.
%and can be implemented by the switch hardware. 
%Note that the presence of nodes with stateful updates makes this problem different from hardware logic synthesis~\cite{SomenziBook}, which is applied mainly to optimize combinational logic (i.e., stateless logic). 
Our code generation procedure is described in Algorithm~\ref{alg:1} and consists of three main steps, each step generating synthesis queries that are solved by SKETCH.

% \vspace*{-0.1in}
\Para{Step 1: Synthesizing stateful updates.} 
First, we consider the stateful updates in $G$. To preserve the packet transaction semantics of the program, each stateful update must be completed in a single pipeline stage, so that the computation finishes by the time the next packet arrives. Thus, it \emph{must} fit within a single stateful ALU, since state cannot be shared across ALUs. For each stateful node in $G$, we generate a SKETCH query to check if the stateful update can be implemented by a stateful ALU, modeled using a SKETCH grammar $A_1$, and assert that the query succeeds. If a query fails, our procedure terminates with an error. 
%as some stateful update cannot fit in the provided stateful ALU.

\begin{figure}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.35\textwidth]{figures/blue_decrease_ex.png}
    \vspace*{-0.1in}
    \caption{Computation graph for BLUE(decrease)~\protect\cite{blue}}
    \label{fig:blue_decrease}
    \vspace*{-0.2in}
\end{figure}

% \vspace*{-0.1in}
\Para{Step 2: Predecessor packing optimization.}
%Packing more into stateful ALUs} 
The stateful update in a single node in $G$ might not fully utilize the available stateful ALU. 
%For example, the Tofino stateful ALU can implement conditional updates for \emph{two} state variables in a single ALU.
%while $C$ may have a separate node for each state variable, leading to separate stateful ALUs being used. 
%Furthermore, if there is an edge between two stateful nodes in $C$, this can lead to an additional pipeline stage that could be avoided.
As an example, %if nodes 2 and 3 in 
consider the computation graph for the BLUE (decrease) example in Figure~\ref{fig:blue_decrease}, where nodes 2 and 3 are stateful updates.
%mapped to separate stateful ALUs in Step 1, resulting in two pipeline stages.
%due to the dependency of node 3 on node 2. 
(In our diagrams, stateful updates are shown in gray-colored boxes and stateless updates in clear boxes; with node numbers shown on the left of the boxes.)
%they will need two stages as node 3 depends on node 2 and must be scheduled after it. 
Here, a single Tofino stateful ALU can actually
%synthesize 
implement both stateful updates in a single stage.
%by mapping each state variable to one of its two registers.
Since pipeline stages are a scarce resource, we would like to reduce the number of stages required by making full use of the switch's ALUs. 
%However, the additional functionality of a stateful ALU can be made use of only if the 
%Therefore, we would like to consider multiple nodes in $C$ and possibly merge them if they fit into a stateful ALU. 
%\xiangyu{The Tofino ALU uses one 64-bit register. We consider the first 32-bit as the first stateful var and the second 32-bit as the second stateful var. I am not sure whether we can mention this details in the paper without violating NDA}

More generally, optimal code generation for a DAG 
%(i.e., for language expressions with common subexpressions) 
is known to be NP-complete~\cite{AJU77}. 
%This problem is also similar to the problem of technology mapping in hardware design, and a practical approach is to partition the DAG into a forest of trees, and solve each tree problem optimally using dynamic programming~\cite{KeutzerDac87}. 
%would require considering all possibilities which would be infeasible for large graphs. Instead, we use a greedy strategy shown in Algorithm~\ref{alg:1}, lines 5 to 11. In reverse topological order, we traverse pairs of adjacent nodes (we ignore nodes with no dependencies as they can be scheduled in parallel) with at least one stateful node, 
%in reverse topological order, 
Here, we use a simple heuristic for optimization, called \emph{predecessor packing}, inspired by similar work in technology mapping for hardware designs~\cite{flowmap}. The main idea is to pack more into a stateful ALU by possibly merging pairs of nodes $u$ and $v$, at least one of which is stateful.
% at node $v$, by possibly merging it with its predecessor node $u$ (which could also be stateful). 
To avoid lengthening other paths in $G$, we only consider a predecessor $u$ that has no other fanouts. 
%\ngs{This sentence made it sound like it was a correctness issue (of affecting other paths), but isn't it an optimality issue? If we can show the example in the appendix, we might rephrase to ``to avoid lengthening any chain of dependencies in $C$ (Appendix XXX),``} 
This is implemented in the function $tryMerge$, which first uses an inexpensive check on the number of inputs and outputs in the combined logic for $u$ and $v$, and then calls a SKETCH synthesis query to check if both can fit into a single stateful ALU.
%This is shown in lines 5 to 11 in Algorithm~\ref{alg:1}, where the function safeToMerge checks if $u$ has no other fanouts, and the function tryMerge checks if $u$ and $v$ can be merged into a single stateful ALU.
% can be merged into the stateful ALU at $v$. 
%In this function (shown in lines 24 to 32), we consider the combined logic $w$ for the updates in nodes $u$ and $v$ (line 25). 
%The function concat on line 25 returns the combination of updates $v_1$ and $v_2$ by concatenating the program statements in the two updates.
% (TODO: explain concat.) 
%We 
%Then, we first use a cheap syntactic check on the number of inputs and outputs (line 26), 
%followed by a Sketch synthesis query (line 27).
%(shown in the function mergeUsingSketch) 
%to check if the merged nodes can fit in a stateful ALU. 
If the query is successful, we merge the two nodes in $G$.
%We repeat the traversal, merging nodes if possible, until 
%a fixed point is reached and 
We apply this process iteratively until no more pairs of nodes can be merged. After convergence, each stateful update in $G$ is \emph{locally maximal} in the sense that it cannot be merged with any predecessor node (with no other fanouts)
and still fit within a stateful ALU. We show the effectiveness of this optimization in our evaluation (\S\ref{ssec:codegen-exp}), where its use results in fewer stages in the solution. 
%\ani{If we can explain the previous paragraph without reference to algorithm 1, we could remove the algorithm listing that is taking up quite a bit of space.}

\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{figures/codegen_example_soln.png}
    \caption{(a) Example computation graph. Outputs to be synthesized are $p.o1$, $p.o2$, and $p.o3$ with corresponding cones of influence $BCI(p.o1) = \{1\}$, $BCI(p.o2) = \{1, 2\}$, $BCI(p.o3) = \{1, 3\}$. (b) Synthesized solution (partial).}
    \vspace*{-0.2in}
    \label{fig:codegen_example}
    % \hfill
    % \begin{subfigure}{0.5\textwidth}
    % \includegraphics[width=\textwidth]{hotnets21-template/Figures/codegen_soln.png}
    % \caption{Synthesized solution.}
    % \label{fig:codegen_example_soln}
    % \end{subfigure}
    % \caption{Example computation graph and synthesized code.}
\end{figure}

% \vspace*{-0.1in}
\Para{Step 3: Minimum-depth solutions for stateless code.} 
After the first two steps, all stateful nodes in $G$ are mapped to stateful ALUs and are locally maximal. We now need to synthesize code for the inputs to these stateful ALUs and the POs of $G$. 
For each variable $o$ to be synthesized, we first compute 
%its specification in terms of PIs and outputs of stateful ALUs (at the end of step 2), by computing 
its backwards cone of influence (BCI), which is often used in verification/synthesis tasks to determine the dependency region (up to some boundary)~\cite{SomenziBook}. In graph-theoretic terms, BCI is the subgraph in $G$ derived by going recursively backward from $o$, stopping at a PI or a stateful node. Essentially, the BCI subgraph provides the \emph{functional specification} for $o$ in terms of PIs and outputs of stateful ALUs. Note that these specifications are stateless since they do not include any stateful nodes. 

We model the switch's stateless ALU functionality also using a grammar, say $A_2$, and then use SKETCH to find a \emph{minimum-depth tree} solution for $o$, where each tree node denotes a stateless ALU allowed by the grammar $A_2$. Since SKETCH cannot directly optimize for minimum depth, we invoke SKETCH in a loop, to find a solution tree of a given depth $i$, %(line 17), 
and iteratively increment $i$ starting from 1. We stop as soon as a solution is found, or if $i$ exceeds the maximum number of pipeline stages. 
%Thus, this step returns a solution tree with the minimum number of pipeline stages. 

% \aarti{maybe we can show only one of the outputs, and put the two figures into one? or skip entirely?} 
% \ngs{I would support showing one output and merging figures given that space is an issue.}
An example computation graph with two stateful updates (gray boxes) and the synthesized solution for one of them is shown in Figure~\ref{fig:codegen_example}; the solution for the second is similar. The stateless updates for $p.o2$ and $p.o3$ need three stages using our algorithm; converting to three-address code, as Domino does, would have required four stages. 
%Although the depth of a solution for each synthesized variable is guaranteed to be minimum, the overall solution might have a larger \emph{width} than required. 
%In our example, 
%in Figure~\ref{fig:codegen_example_soln} 
%note that the updates 
%Although $p.o2$ and $p.o3$ share the update to $p.o1$ (node 1); however, the synthesized solution 
%might not have shared code 
%does not, since separate Sketch queries are used for outputs $p.o2$ and $p.o3$. We leave the synthesis of solutions \emph{with sharing} to future work.
% We leverage min-depth tree algorithm to do code generation for each action portion. At a really high level, the goal of using min-depth tree is to generate code with minimum number of stages for one given program. The whole algorithm can be divided into several stages. The first three stages, which aims at building dependency graph after parsing the input program, are similar to what Domino compiler has done. However, since naively using the dependency graph generated from the first three steps might be unnecessarily large in terms of the depth of that tree, in order to make the tree more compact, the remaining steps are implemented in sequence. Based on the generated dependency graph, step 4 tries to separate SCCs from WCCs since we will use different procedures for code generation. As for SCCs, a single SKETCH is used to check whether a stateful ALU can implement the stateful update or not, while as for other WCCs, we treat each component as the specification and a grammar, which captures the switch functionality and is parameterized by an integral bound, is considered as implementation. Given a bound of depth, SKETCH is used to check whether there exists an implementation that can fully express the given input program. Since the bound starts from one and we increment the bound by one each time, this procedure is capable of finding the expression tree of minimum depth that satisfies the specification. With the generated code in hand, step 6 combines the results from SCCs and WCCs by preserving their dependency relationships. Finally, the last step, optimization step, checks the possibility of merging adjacent nodes of stateful super nodes to eliminate more components by fully utilizing the additionaly functionality from stateful ALU on top of the stateful updates. The final optimization step offers a second chance to reduce the total number of depth of our generated code.

\subsubsection{Correctness and Optimality of Code Generation}
The final result of all three steps in code generation is in the form of a resource graph $R$, where each node $v$ is mapped to either a stateful or a stateless ALU, and an edge $(u, v)$ indicates that an output of the ALU at $u$ is connected to an input of the ALU at $v$. 
%The PIs, POs, and state variables in $R$ are the same as in $C$. 
Due to the guaranteed correctness of program synthesis in SKETCH over a bounded input range, the POs and stateful updates in $R$ are guaranteed to be functionally equivalent to those in $G$ for the same input range. The predecessor packing in Step 2 results in locally maximal use of stateful ALUs, and the min-depth tree solutions in Step 3 are optimal in using a minimum number of stages with stateless ALUs. Note also that each SKETCH query in our procedure is smaller than a query for the full transaction, thereby resulting in significant performance improvement overall, as demonstrated later in our evaluation (\S\ref{sec:eval}).

%In terms of comparison, the Chipmunk compiler~\cite{chipmunk} also supports transactions, but it invokes program synthesis on an \emph{entire transaction scope} in an individual synthesis query, which leads to long and variable synthesis times, even with a slicing-based technique.
%that creates smaller subproblems for synthesis. 
%In contrast, our approach separates the synthesis of stateful updates from stateless updates, since the former are critical for successful code generation, and the latter queries are over possibly smaller subgraphs that comprise stateless logic regions between stateful updates\footnote{This is inspired in part by logic synthesis in hardware design~\cite{SomenziBook}, which optimizes  combinational logic between stateful updates.}. 
%As shown later in our evaluation (\S\ref{sec:eval}), our compiler achieves 
%the same minimum number of pipeline stages 
%comparable quality of results as Chipmunk, but with significant speedup in runtimes. 
%Another big difference is that Chipmunk does not consider multiple transactions or pack them in the pipeline stages.

\subsection{Constraint-based Resource Allocator}
\label{ssec:resource_allocation}

The second phase of our compiler uses a
%integer linear programming (ILP) 
constraint-based formulation
to allocate resources such as 
memory blocks and ALUs for P4 language constructs such as tables and expressions.
% , and registers. 
The constraints for memory blocks are similar to prior work by Jose et al.~\cite{lavanya_nsdi15}. In addition to Jose et al.'s formulation, we formulate constraints for ALUs.
% and table resources.
%One distinctive feature of our formulation is that 
We aim to allocate resources for \emph{multiple actions} in each pipeline stage 
as long as the corresponding computations have no dependencies, which we identify from a table dependency graph (similar to prior work~\cite{lavanya_nsdi15,cetus}). Moreover, unlike prior work~\cite{lavanya_nsdi15,cetus}, our formulation can handle multi-stage actions as well as atomic transactions. 
We use the resource graph $R$ derived for each action (after code generation) to enforce {\em intra-table constraints}, and use the table dependency graph to enforce {\em inter-table constraints}. In the remainder of this section, we describe our resource allocation constraints with reference to a generic RMT design; these can be easily extended to other hardware resources in a specific architecture.
%Our formulation extends Jose et al.'s formulation~\cite{lavanya_nsdi15} with constraints over ALUs.

\Para{Constants.} We use the following constants:
%in our formulation:
%to represent maximum limits on hardware resources: 
\begin{CompactItemize}
    \item 
$N_S$ denotes the maximum number of pipeline stages.       \item 
$N_{alu}$ denotes the maximum number of ALUs in each stage (could be generalized to be different per stage).
    \item 
$N_{table}$ denotes the maximum number of logical table IDs per stage.
    \item 
$N_{entries}$ denotes the maximum number of match entries per table in each stage.
    \item 
For table $t$, we use a constant $e_t$ to denote the %maximum% 
number of match entries in the table, as specified in the program.
\end{CompactItemize}

\Para{Handling tables with too many entries.} If a table $t$ has too many entries ($e_t > N_{entries}$) to fit within a single stage, we partition these entries into $b_t$ separate tables that can each fit within a single stage, where $b_t = \lceil(e_t/N_{entries})\rceil$. If the match type is exact, a packet will match at most one of these $b_t$ tables, and they can be regarded as independent tables with the same actions as table $t$. Our partitioning procedure could be extended in the future to support other types of matches.

\Para{Handling multi-stage actions.} We handle a multi-stage action under the condition that it 
%Assuming that a multi-stage action 
does not modify the table's match key, by duplicating the match entries at each stage to ensure that the entire action is executed. For example, suppose match entry $m$ in table $t$ is associated with action $A$ that takes 2 stages, $s_1$ and $s_1 + 1$. We allocate table $t$ in both stages $s_1$ and $s_1 + 1$. If a packet matches entry $m$ in table $t$ in stage $s_1$, it will match entry $m$ in table $t$ in stage $s_1 + 1$ as well, resulting in action $A$ being executed completely. 
If Action $A$ is allocated to non-consecutive stages, we allocate additional ALUs in the intermediate stages
%duplicate the match entries in each intermediate stage\xiangyu{Actually, we do not duplicate the match entries in all intermediate stages. We only duplicate in stages that ALUs belonging to that action appear}, using ALUs (\hl{AG: this seems specific to FPGAs, should we mention that other PISA architectures could use PHVs?}) 
to propagate the intermediate results to the next stage. Note that Menshen requires additional ALUs for propagation of intermediate results; other RMT architectures could use, for example, dedicated ``tag-along'' PHV containers for propagating intermediate results. Thus, propagation constraints apply to either ALUs or to PHV container resources, depending on the specific architecture. Note that with PHVs, these constraints would allow sharing of PHVs for variables with different lifetimes.

\Para{Variables.} 
% integer variables $S_t$ and $E_t$ denoting the starting and ending stages allocated to the table (as a design decision, we choose to allocate each table in consecutive stages), and
% an integer variable $M_{ts}$ denoting the number of memory units in stage $s$ allocated to the table.
For the $a^{th}$ action in the $i^{th}$ partition of table $t$, we use $R_{tia} = (V_{tia}, E_{tia})$ to denote the corresponding resource graph which is computed in the code generation phase. Recall that this resource graph could span multiple stages. For each partition $i$ of table $t$, we use a binary variable $M_{tis}$ which is $1$ if the match part of the table is assigned to stage $s$, and $0$ otherwise. We use an integer variable $stage_{u}$ to denote the stage assigned to ALU $u$, and a corresponding binary variable $stage_{us}$ which is $1$ if ALU $u$ is assigned to stage $s$ and $0$ otherwise.

We define $I$ to be the set of ALUs whose outputs are intermediate variables (i.e., temporary packet fields or read or write flanks of state variables), and $R_u$ to be the set of ALUs that read the output of ALU $u$. These sets are computed by analyzing the resource graph of each action. For each ALU $u$ in $I$, we use an integer variable $beg_u$ to denote the stage the computation is performed and an integer variable $end_u$ which is at least as large as the last stage where the output of ALU $u$ is used. For each ALU $u \in I$, we use a binary variable $prop_{us}$ which is $1$ if an additional ALU that propagates the result of ALU $u$ to the next stage is assigned to stage $s$, else $0$.


\Para{Constraints.}
We now describe the constraints in our formulation. We begin with constraints related to allocation of table entries, and dependencies between tables. These extend the formulation in prior work~\cite{lavanya_nsdi15} by dealing with actions, where actions can possibly span multiple stages. 
% (similar to prior work~\cite{lavanya_nsdi15}). 
%except we abstract away some details of memory allocation.

%\noindent
% \paragraph{Memory allocation constraints.}  For each table, the total number of memory units allocated must be at least as large as the number of table entries.
% \begin{equation*}
%     \sum_s M_{ts} \geq e_t 
% \end{equation*}

\Para{Match constraints.} For every ALU assigned to a stage, its corresponding match entries must also be assigned to that stage.
\begin{equation*}
    \forall s \ \forall t, i, a \ \forall u \in V_{tia}: \ \ \ stage_{us} = 1 \rightarrow M_{tis} = 1
\end{equation*}

\noindent
\Para{Table dependency constraints.}
We consider four types of table dependencies: match, action, successor, and reverse-match~\cite{lavanya_nsdi15}.
If table $t_2$ depends on table $t_1$, all ALUs of $t_2$ are allocated after ALUs of $t1$. For successor and reverse-match $<$ below should be replaced by $\leq$.
\begin{align*}
    & \forall i_1, i_2, a_1, a_2, \forall u_1 \in V_{t_1\ i_1\ a_1}, \ \forall u_2 \in V_{t_2\ i_2\ a_2}: \\
    & stage_{u_1} < stage_{u_2}
\end{align*}
%\hl{AG: do we need forall u2 in above?}\xiangyu{Yes, we do need forall since we only care about action level dependency rather than ALU level dependency. Based on our constraints, if it is match/action dependency, it is $stage_{u1} < stage_{u2}$ while as for successor/reverse dependency, it should be $stage_{u1} \leq stage_{u2}$}

\noindent
\Para{Action dependency constraints.} The allocation of ALUs to stages must respect the dependencies within an action, given by the edges of the corresponding resource graph $R_{tia}$. If the output of ALU $u$ is an input of ALU $v$, then $u$ must be allocated in an earlier stage than $v$.
\begin{equation*}
    \forall t, i, a \ \forall (u, v) \in E_{tia}: \ \  stage_u < stage_v
\end{equation*}

\noindent
\Para{Propagation constraints.} If ALU $v$ depends on ALU $u$ and they are not allocated in consecutive stages, we allocate additional ALUs to propagate the output of ALU $u$ until the stage assigned to ALU $v$.
% \hl{AG: using an ALU for propagation seems specific to the FPGA, should we note that PHV containers could be used in other architectures?}

The output of $u$ is computed in $stage_u$, and $beg_u$ must be less than $end_u$.
\begin{align*}
   &\forall u \in I: \ \ beg_u = stage_u\\
   &\forall u \in I: \ \ beg_u < end_u
\end{align*}
Variable $end_u$ must be as large as the stage assigned to any ALU $v \in R_u$ that uses the result of ALU $u$.
\begin{align*}
    &\forall u \in I, \forall v \in R_u: \ \ end_u \geq stage_v\\
    &\forall u \in I: \ \ end_u \leq N_S
\end{align*}
For all stages $s$ where $beg_u < s < end_u$, we must allocate an ALU to write the output of $u$ to the next stage.
\begin{equation*}
    \forall u \in I, \forall s \in \{1,\ldots,N_S\}: \ \ (beg_u < s \land s < end_u) \leftrightarrow prop_{us} = 1
\end{equation*}
If an ILP solver is used, the above constraints can be formulated using the well-known Big-M method, as shown in Appendix~\ref{appendix:bigm_encoding}.

\noindent
\Para{Resource constraints.}
The stage allocated to each ALU must be within the range of available stages.
\begin{equation*}
    \forall t, i, a \ \forall u \in V_{tia}: \ \ 1 \leq stage_{u} \leq N_S\\
\end{equation*}
The number of ALUs allocated in each stage must be less than or equal to the number of ALUs available, $N_{alu}$. We allocate $H$ ALUs per stage to transport the packet header fields through the pipeline. We need to make sure that the number of ALUs for intermediate fields
%\xiangyu{and stateful variables. (Because stateful ALUs also need allocation)} 
is no more than $N_{alu} - H$.
Note again, that the $H$ constraint is specific to our FPGA platform that uses ALUs for propagation (as described earlier); other architectures need not use ALUs for propagation. 
%\hl{AG: again, isn't this specific to the FPGA?}\xiangyu{This should be substrate-specific to this FPGA design}
\begin{align*}
&\forall s\ \forall t, i, a,\ \forall u \in V_{tia}:\ \  stage_{u} = s \leftrightarrow stage_{us} = 1\\
&\forall s\ \forall u \in I: \ \  stage_{us} + prop_{us} \leq N_{alu} - H
\end{align*}
Finally, the number of tables allocated in a stage must be less than or equal to the number of table IDs available, $N_{table}$.
\begin{equation*}
    % \forall s \in \{1, \ldots, N_S\} \sum_{t, i} I(\bigvee_{u \in V_{ti}} stage_u == s) \leq N_{table}
    \forall s: \ \ \sum_{t, i} \ \ M_{tis} \leq N_{table}
\end{equation*}

\noindent
\Para{Solving the constraint problem.}
We can use either an ILP solver (Gurobi~\cite{gurobi}) or an SMT solver (Z3~\cite{z3}) to find either an optimal or a feasible solution, depending on the choice made by a user. (Note that Z3 supports optimization with the theory of linear integer arithmetic.)
 %\xiangyu{In the ILP file, we allow users to set the mode flag. The default mode is optimization while if they set it to feasibility on purpose, the ILP solver will output one feasible solution.}
%\noindent
%\paragraph{Optimality constraints.} 
\begin{itemize}
    \item Optimality constraint: 
If the user chooses to find an optimal solution, they can optionally specify an objective function. For example, one can minimize the number of stages occupied, since this is often the most scarce resource within a switch. Formally, the objective function is $\min\ cost$ where $cost$ is greater than or equal to the stage assigned to every ALU: $\forall t, i, a,\ \forall u \in V_{tia}:\ cost \geq stage_u$.

% \hl{AG: please add a small para on finding a feasible solution below.}
%\noindent
%\paragraph{Feasibility constraint.}
\item Feasibility constraint: 
If the user opts to find a feasible (but not necessarily an optimal) solution, we use a trivial objective function such as $min\ 1$ with Gurobi. With Z3, we omit an optimization function, and simply let it find a feasible solution.
\end{itemize}
%\hl{AG: Instead of above para on Feasible solution, add a para on "Solving the Constraint Formula" and describe how we can use either Gurobi or Z3 to find either an optimal or a feasible solution.}\xiangyu{In the ILP file, we allow users to set the mode flag. The default mode is optimization while if they set it to feasibility on purpose, the ILP solver will output one feasible solution.}

\iffalse
The result of the code generation phase is a resource graph for each action in the P4 program. We denote the resource graph for the $i^{th}$ action in table $t$ by $R_{ti}$. The resource graphs of non-atomic actions consist of a single node representing the ALU which implements the update. %\aarti{please explain -- is such an action a single update? We would have checked that it fits, right?}
Due to space limitations, we describe allocation of ALUs from resource graphs for actions; handling memory blocks is similar to prior work~\cite{lavanya_nsdi15}.

Given these resource graphs, one for each P4 action, the second phase of our compiler uses an ILP to pack the resource graphs into the switch's pipeline stages so that they take the minimum number of stages, while respecting the dependencies %between nodes 
in each resource graph as well as the dependencies between tables. The objective function of the ILP minimizes the total number of stages, and the constraints encode the resource constraints of the switch and the dependencies between resources. 
% We specify the objective function and describe how to encode chip-specific constraints for our ILP scheduler based on our best-effort understanding of the Tofino switch. These constraints are the key determinant for our final ILP optimization problem. 
\iffalse %%AG moving this to later, after the constraints
\Para{Objective function} We use an objective function that minimizes the total number of stages occupied since this is the most scarce resource within a switch. Formally, the objective function is $\min cost$
% where for all tables $t$ and all ALUs $i$, $cost \geq t\_Act\_i$ where $t\_Act\_i$ is the stage assigned to the ith ALU of table $t$.
where for all tables $t$, all actions $i$, and all nodes $u \in R_{ti}$, $\ cost \geq stage_u$, with $stage_u$ denoting the stage number assigned to node $u$.
% Why does optimization matter (relative to satisfiability) on all-or-nothing line rate?
\fi %%AG end of iffalse
%\paragraph{ILP Constraints}
%\subsubsection{ILP Constraints} 
There are two main types of constraints in our ILP formulation: resource constraints and dependency constraints.
%\aarti{what about memory block constraints -- we should say something even if our benchmarks didn't use any.}

\noindent
\textbf{Resource constraints.} For each ALU $u$ in each resource graph, we define 
% $n$ as the total number of ALUs required for its actions and
$stage_u$ as the stage number allocated to it. We define $N_{alu}$ as the total number of ALUs available per stage and $N_{table}$ as the total number of logical table IDs per stage. The resource constraints are encoded below, where $I(c)$ is an indicator variable that is equal to $1$ if condition $c$ is true and $0$ otherwise.\\
$\forall s, \sum_{t, i} \sum_{u \in R_{ti}} I(stage_u == s) \leq N_{alu}$.\\
% $\forall s, \sum_{t, i} I(t\_Act\_i == s) \leq N_{table}$.\\
%$\forall s, \sum_{t, i} \sum_{u \in R_{ti}} I(stage_u == s) \leq N_{table}$.\\
$\forall s, \sum_{t, i} I(\bigvee_{u \in R_{ti}} (stage_u == s)) \leq N_{table}$.\\
%\todo{check: isn't this counting each action in each table?}
%\aarti{please explain what is denoted by I(.). The second constraint doesn't seem correct -- if two ALUs from action of the same table are assigned to stage s, this should still be counted as only 1 table -- you should not sum over ALUs from the same table for checking against N\_table}
%\xg{Hi Aarti, this is an issue of our current setting. When we divide one atomic action block into multiple ALUs, we need to put each ALU into one new table so as to implement its functionality. Therefore, we need to sum over ALUs from the same table. But maybe we need to clarify this point to avoid any misunderstanding.}
%\ngs{I too got tripped up by the second constraint above, like the others seem to have. }

\noindent
\textbf{Dependency constraints.} 
In addition, the solution must respect the dependencies between logical tables (inter-table dependencies) and within each logical table (intra-table dependencies). 
If table $t_{2}$ depends on table $t_{1}$, then any ALU of $t_{2}$ is allocated \emph{after} any ALU of $t_{1}$, using the following constraint:
%To be specific, if table $t_{2}$ depends on table $t_{1}$, then any ALU of $t_{2}$ should be allocated \emph{after} any ALU of $t_{1}$: \ngs{Should it? It depends on which ALU induced the table-level dependency, no? May rephrase as ``we use the following constraint to allocate any ALU of t2 after any ALU of t1''}\\
% if $t_{2}$ depends on $t_{1}$, $\forall i, j, t_{1}\_Act\_i \leq t_{2}\_Act\_j$.\\
$\forall i, j \ \forall u1 \in R_{t1i}, u2 \in R_{t2j}, \   stage_{u1} < stage_{u2}$.\\
The intra-table dependencies are given by the edges of the resource graph for each action in a table.
% As for all ALUs generated for action in a specific table $t$, in order to preserve the semantics, the resource allocation for them must be consistent with the order from code generator.
% If $t\_Act\_i$'s output is an input of $t\_Act\_j$, then we must allocate $t\_Act\_i$ to in an earlier stage than $t\_Act\_j$:\\
% for table $t$, if $ALU_{j}$ depends on $ALU_{i}$, $t\_Act\_i \leq t\_Act\_j$
If node $u$'s output is an input of node $v$, then $u$ must be allocated to an earlier stage than $v$.
For each resource graph $R_{ti} = (V_{ti}, E_{ti})$,
$\forall (u, v) \in E_{ti}, stage_u < stage_v$.
% ILP technique used to encode various constraints
% Constraint 1: # of available ALUs per stage
% Constraint 2: # of available tables per stage
% Constraint 3: inter-table dependency (table level dependency)
% Constraint 4: intra-table dependency (action level dependency)

%\paragraph{Objective function}
%\subsubsection{ILP Objective Function}
\noindent
\textbf{ILP Objective Function.}
We use an objective function that minimizes the total number of stages occupied since this is the most scarce resource within a switch. Formally, the objective function is $\min cost$
% where for all tables $t$ and all ALUs $i$, $cost \geq t\_Act\_i$ where $t\_Act\_i$ is the stage assigned to the ith ALU of table $t$.
where for all tables $t$, all actions $i$, and all nodes $u \in R_{ti}$, $\ cost \geq stage_u$.
% with $stage_u$ denoting the stage number assigned to node $u$. (defined previously).
% Why does optimization matter (relative to satisfiability) on all-or-nothing line rate?

\fi 

%\subsection{Combination of both generator and allocator}
%\subsection{CaT Compiler Workflow}

==> design.tex <==
\section{Compiler Design}
\label{sec:design}
Our main approach is centered around decomposing the overall compilation problem into: (1) code generation: to map each action-computation in the program to hardware resources based on its functionality, and (2) resource allocation: to pack resources for all computations and all data structures in all tables to available hardware resources based on resource constraints. Unlike existing compilers, we allow actions where computations may need ALUs in more than one stage---this is needed for allowing rich actions that employ atomic transactions~\cite{domino} and actions that have dependencies between their constituent statements. Effectively, our compiler explores the space of semantically-equivalent program transformations for actions during code generation. 

\subsection{HLS-Inspired Modular Decomposition}
\label{ssec:hls}
The modular decomposition in our compiler approach is inspired by the success of HLS techniques in development of software-hardware systems in modern Systems-on-Chip (SoC) design~\cite{hls}. Starting from a high-level algorithmic description of a hardware component, an HLS tool performs various steps to ultimately generate a lower-level hardware design for an FPGA or ASIC, usually cycle-accurate at the register-transfer level (RTL). These steps include compiling the specification to a (typically) graph-based intermediate representation, \emph{allocating} resources (functional units, storage, buses, etc.), \emph{scheduling} the operations to clock cycles, \emph{binding} the operations to functional units, \emph{binding} the variables to storage elements and transfers to buses, and generating the final clock-accurate RTL design.

In our context, we regard the specification as a P4-16 program and lower it to hardware in the RMT architecture, taking into account the available resources (ALUs, memory, tables, packet header vectors (PHVs), etc.) in pipeline stages. Our code generation procedure can be viewed as finding a schedule for the required operations on the available functional units, while our resource allocation procedure can be viewed as binding the operations/variables/transfers to resources in specific stages of the pipeline. 

Note that we perform code generation \emph{locally}, i.e., for each computation in each table, which keeps the synthesis runtime manageable in practice, even when we use program synthesis to explore the space exhaustively (as shown in \S\ref{sec:eval}). These independent code generation tasks could be parallelized in a future implementation.
%In our current approach, we do not allow these computations to share any resources, e.g., for stateful updates. In future work, we plan to consider static analyses of P4 programs to group together computations that can potentially share resources. Each such group can then form a local unit on which code generation is performed simultaneously. 
On the other hand, we perform resource allocation \emph{globally}, i.e., by considering all computations in all tables in the program. 
%Note that this is enabled by the earlier code generation step, which determines the resources required for each individual computation. When considering packing computations from different tables into the available pipeline stages, our prototype compiler enforces table-level dependencies. This allows computations of independent tables to be potentially packed into the same stage of the hardware pipeline. Our approach can be extended straight-forwardly to pack computations at a finer granularity of operation-level dependencies in future work. 

Our modularization of the compilation problem into local code generation followed by a global resource allocation can be viewed as decomposing the overall problem into smaller subproblems.
%where the local subproblems find solutions to ensure that computations can be mapped to available resources based on functionality, and the global step ensures that all local solutions can be packed into available resources based on capacity. 
This decomposition has the following benefits, in contrast to an alternative approach that would perform code generation and resource allocation \emph{simultaneously} on the full problem. 
\begin{CompactEnumerate}
    \item When performing code generation on small local subproblems, the search space over semantically-equivalent code is smaller, thereby resulting in reasonable performance when using program synthesis (\S\ref{sec:eval}). 
    \item The small subproblems allow us to perform optimization during code generation. In particular, for each subproblem, we find a solution that has a locally minimal depth, i.e., number of pipeline stages. Since the pipeline stages are often a critical resource, the optimized local solutions make it more likely that the global step for packing them based on capacity will succeed. 
    \item It provides the flexibility of looking for a feasible (in addition to an optimal) solution in the global packing step, where the available capacity of hardware resources (e.g., number of pipeline stages) is known. Note that looking for feasible solutions for local subproblems would require guessing suitable hardware capacity limits at the local level, which are not fixed, and too loose or too tight guesses may result in overall compilation failure. Thus, our decomposition enables combining good performance and optimality in local synthesis solutions, with feasible or optimal packing at the global level.
\end{CompactEnumerate}

The general problem of optimal code generation in compilers is known to be NP-complete~\cite{AJU77}, and most compilers decompose the problem in some way to tradeoff optimality for reasonable performance. 
In HLS too, although the tasks to be scheduled are inter-dependent, they are often performed in some sequence to manage the computational complexity of synthesis~\cite{hls}.
%Note that our code generation procedure is applied to one transaction at a time, which keeps the runtime manageable in practice (as shown in \S\ref{sec:eval}). 
%The resource allocation is performed only once for the global P4 program, which allows pipeline stages to be utilized maximally among transactions that are independent. Thus, 

Our approach can be viewed as an \emph{action-level decomposition}, where we perform local code generation for each computation, and then use these results to perform a global resource allocation
for multiple computations. %where multiple computations can be packed within a single stage of the pipelined architecture.
In future work, we plan to perform additional static analyses of P4 programs: to group together computations that can potentially share resources, and to identify operation-level dependencies at a finer level of granularity than table-level dependencies. Each such group can then form a local unit on which code generation is performed, and we can consider operation-level dependencies to further improve packing during resource allocation. 

%This scheme provides an effective transaction-level decomposition of the compilation problem. 
%This transaction-level decomposition is another contribution, providing a crucial first step in building compiler support for transactions.
%For code generation, we provide local optimality guarantees within each transaction (\S\ref{sec:codegne}; for resource allocation, our ILP-based method (\S\ref{sec:ilp}) provides optimality for the target cost. 
%The purpose of code generation is to map each node in $C$ to some hardware resource, e.g., a stateless/stateful ALU, such that the outputs and state updates are implemented correctly. 
%\subsection{High-level overview}
%Our compiler consists of two main phases. In the first phase, we perform \emph{code generation} for each transaction in the P4 program.
%, starting from a \emph{computation graph} $C$ that represents the transaction as a graph of dependencies. 
%The result of our code generation is a \emph{resource graph} $R$, where each node is a hardware resource (e.g., an ALU), and an edge $(u,v)$ denotes that the output of $u$ is connected to the input of $v$. 
%Like the Chipmunk compiler~\cite{chipmunk}, our code generator also leverages automated program synthesis~\cite{sketch,AlurSygus} to exhaustively search over the space of target programs without depending on rewrite rules.
%, but there are significant differences (described later). 
%Given a specification and a grammar, the Sketch tool~\cite{sketch} synthesizes a correct program allowed by the grammar. 
%Our code generation procedure is guaranteed to be correct and we discuss the conditions under which it is optimal.
%in terms of number of pipeline stages.

%available in the hardware pipeline. 
%We identify such independent transactions by analyzing the dependency relations between the tables in the P4 program.
%\todo{add a sentence on the type of table dependencies, and when tables are triggered.} 
%The second phase of our compiler performs \emph{resource allocation} based on integer linear programming (ILP), to allocate resources such as memory blocks and ALUs for P4 language constructs such as tables, expressions, and registers. 
%The constraints for memory blocks are similar to prior work by Jose et al.~\cite{lavanya_nsdi15}. In addition, we consider constraints for other resources, such as ALUs, informed by the resource graphs generated by the code generation phase. 
%The main idea is to allow allocation of resources for \emph{multiple transactions} in each  pipeline stage, as long as the corresponding transactions have no dependencies, which we identify from a table dependency graph similar to that proposed by Jose et al.~\cite{lavanya_nsdi15}.
%Thus, we use the resource graph $R$ of each transaction to enforce {\em intra-table constraints} in the ILP, and use the table dependency graph to enforce {\em inter-table constraints}.
%node resource allocation constraints and input-output connection constraints. The latter kind of constraint enforces that the output of a resource allocated in some stage $i$ is connected as an input to another resource allocated in some stage $j$, where $j > i$, i.e., we do not require $j$ to be $i+1$ necessarily. \emph{This provides flexibility on top of code generation alone, to enable packing the resources for multiple transactions in each pipeline stage.} We can add capacity constraints, such as number of available ALUs per stage, or total number of pipeline stages, and we can optimize with different (linear) objectives, e.g., to minimize the number of pipeline stages or the total number of resources, etc.
%\ani{We could comment out the para below if we are out of space.}
%Aside from novelties in our code generation and resource allocation procedures, we believe that our decomposition of the overall compilation problem into these two phases is also a distinct contribution. 
%The general problem of optimal code generation in compilers is known to be NP-complete~\cite{AJU77}, and most compilers decompose the problem in some way to tradeoff optimality for reasonable performance. Note that our code generation procedure is applied to one transaction at a time, which keeps the runtime manageable in practice (as shown in \S\ref{sec:eval}). (These code generation tasks could be parallelized in a future implementation.) 
%The resource allocation is performed only once for the global P4 program, which allows pipeline stages to be utilized maximally among transactions that are independent. Thus, 
%Effectively, we use the results of \emph{local} per-transaction code generation to perform a \emph{global} transaction-level packing in resource allocation. 
%This scheme provides an effective transaction-level decomposition of the compilation problem. 
%This transaction-level decomposition is another contribution, providing a crucial first step in building compiler support for transactions.
%in packet-processing applications.

%The following subsections describe details of our code generation and resource allocation procedures, along with the compiler workflow that combines them.
% TODO: use one concrete example figure to show how min-depth tree works
% TODOs: min-depth tree example
We consider each individual action in a program, where action computations are not restricted to a single stage, i.e., we can handle computations that may require multiple stages in the pipeline. In addition, we consider computations with atomic transactional semantics~\cite{domino}, i.e., where stateful updates are required to be performed in a single stage within the pipeline to guarantee atomicity. In the remainder of the paper, we refer to these general action-computations as \emph{transactions}.

For a given transaction, we use the SKETCH~\cite{sketch} program synthesis tool to generate \emph{semantically equivalent} code, similar to Chipmunk~\cite{chipmunk}. We note two important differences from Chipmunk.
%of our code generation procedure. 
%for a programmable switch target. 
First, we aim to reduce code generation time by creating \emph{smaller synthesis queries} for SKETCH, rather than invoking it for synthesis of the entire transaction as done in Chipmunk. To mitigate the narrower scope of search in smaller synthesis queries, we perform additional optimizations. Second, %similar to Chipmunk, 
rather than Chipmunk's approach of creating low-level holes in the ALU grid architecture that are filled by SKETCH, 
our code generation procedure is \emph{parameterized by the grammar} that is used by SKETCH in the synthesis queries. 
This enables the same code generation procedure to be used for different hardware backends via grammars. Our compiler currently supports three different grammars: Tofino ALUs~\cite{tofino}, Banzai ALUs~\cite{domino}, and ALUs for our simulation of Menshen~\cite{menshen}; more can be supported as needed without modifying our overall procedure.
%First, the P4 action is converted to an equivalent Domino program which is then transformed using multiple phases, each of which is described below.
The rest of this section describes the steps of our preprocessing optimizations and code generation procedure in detail. 

\begin{figure}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.5\textwidth]{figures/Preprocessing-CFG.pdf}
    \vspace*{-0.1in}
    \caption{The control flow graph (right) of a P4 control block (left), simplified from the SipHash example \ruijie{Can someone please add citations for SipHash example here? thanks}. WAW dependencies shown as dotted red edges. Here $v1\neq v2 \neq v3$ are integer constants.}
    \label{fig:p4cfgcb}
    \vspace*{-0.2in}
\end{figure}
\begin{figure}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.5\textwidth]{figures/Preprocessing-Canonicalization.pdf}
    \vspace*{-0.1in}
    \caption{Illustration of the canonical form for preprocessed P4 programs; program A is from Figure \ref{fig:p4cfgcb} and program B taken from the UPF Rate\_enforcer example \ruijie{can someone please add citations here for the UPF example? thanks}. Packet fields in if conditionals highlighted in blue and newly created actions highlighted in orange.}
    \label{fig:p4Canonical}
    \vspace*{-0.2in}
\end{figure}



\subsection{Preprocessing of a P4 program.}
First, we do preprocessing of the entire input P4 program to perform a dependency-based early optimization of the input program by canonicalizing the table dependencies specified in the P4 control block.

The sequence of program statements inside the \texttt{apply \{...\}} block of a P4 control block can be treated as a straight-line program with (possibly nested) if-statements, reads and writes to packet header vector (PHV) fields, and \texttt{apply} statements, which apply match-action tables. The program statements inside a control block, altogether with table applies, induce Read-after-Write (RAW), Write-after-Read (WAR), and Writer-after-Write (WAW) dependencies between pairs of variables at different program locations. These dependencies, in turn, become hard resource scheduling constraints during resource allocation. Conventionally, RAW, WAR and WAW dependencies are defined between pairs of program locations without taking into account of path information of program control flow, where $v$ at program locations $l_1$ and $l_2$ form a depedency pair $(v@l_1\to v@ l_2, t)$ for $t\in \{RAW,WAR,WAW\}$. However, this is a conservative notion of dependency; consider the example provided in Figure~\ref{fig:p4cfgcb}. In this example, although WAW dependencies exist between program locations suggesting that any realization of this program takes 3 pipeline stages, \emph{no real dependencies exist} as the if conditionals containing them are disjoint, thus the program can be implemented in a single pipeline stage. We have found that in practice, popular P4 compilers (p4c and the Tofino compiler) employ the use of the conservative, syntax-based dependency analysis without taking into account path information provided by program control flow, thus producing compilation results that are suboptimal in terms of pipeline usage.

\subsubsection{Guarded dependency analysis.} To solve the aforementioned issue, we refine the notion of RAW/WAR/WAW dependencies between program locations into \emph{guarded dependencies} that take into account path condition of program control flow, and describe a canonical representation of the P4 program's control block as a straight-line sequence of match-action table applies that allows us to encode precise dependency information in the program structure in a form such that when the Tofino and p4c compilers can rediscover only the true dependencies when supplied with the canonicalized program. The refined notion of dependencies allows us to \emph{prune out} overapproximate program dependencies by deciding path reachability using an SMT-solver. The input program is then rewritten to our caninical form, which enables conventional P4 compilers to rediscover the precise dependencies.

Given the control-flow graph $G$ for a P4 control block, a \emph{guarded dependency} between nodes $(u,v)\in G$ is a tuple $(\phi,v@l_1\to v@l_2,t)$ where $v$ is the variable of concern,  $t\in\{RAW,WAR,WAW\}$ and $\phi$ is a conditional that describes the condition under which node $v$ may be visited after node $u$ is visited. As we show below, the condition $\phi$ is be computed by lightweight static analysis of the program control-flow. The infeasible dependencies (dependencies where $\phi$ is unsatisfiable) can then be discovered using an SMT solver and removed.

\subsubsection{Canonicalization.} We define the canincalized representation of a P4 control block to be such that every statement inside the \texttt{apply\{ ...\}} block is a match-action table application. The entire control block therefore consists only of match-action tables, and free of if-then-else and assignment statements. Figure~\ref{fig:p4Canonical} provides an illustrative example of two P4 programs pre- and post-conversion into canonical form. Canonicalizing the program into a sequence of match-action table apply statements allows us to explicitly encode the data dependencies in the control flow discovered by the guarded dependency analysis.

\subsubsection{Performing the guarded dependency analysis.} We now describe a static analysis procedure to compute guarded dependencies. First, we make some assumptions about the control flow graph $G$ of a P4 control block. We first make the standard assumption the graph is \emph{well-structured} (i.e., no go-tos), so that only the basic blocks at merge points of branches have multiple edges coming in. We additionally assume that none of the assignment statements update any variables in conditions; the reason is that if assignment statements update any variables in conditions, there would be RAW dependencies which we cannot remove, so we would quit. 

With these assumptions, the path condition under for program statements are simple conjunctions on branch conditions, as the disjunction at merge points will disappear, and the branch condition variables are never updated. An example is illustrated in [figure ??] 
\ruijie{TODO to self: add in small example illustrating this}. Then, for a pair of nodes $(u,v)\in G$, the corresponding path condition $\phi$ is just the path condition for $u$, conjuncted with the path condition for $v$.

\subsubsection{Preprocessing of a P4 action block.} 
We do preprocessing per action block of the P4 program to prepare each action block for synthesis-based code generation. We use some standard preprocessing steps similar to the Domino compiler~\cite{domino} on the P4 code for a given transaction. In the branch removal step, conditional expressions (if statements) are replaced by conditional assignments to produce straight-line code. Then, for each stateful variable in every transaction, we create two temporary packet fields, \emph{pre-state packet field} and \emph{post-state packet field}), which store the initial and final values of state variables. The pre-state field stores the pre-transaction value of the stateful variable, and the post-state field stores the post-transaction value of the stateful variable; see Figure~\ref{fig:statefulALU} for illustration. Altogether, the pre-state and post-state fields guarantee the stateful transactions are represented as strongly connected components in the resultant graph created from read-after-write and write-after-write dependencies between packet fields and stateful variables.\footnote{The notion of pre/post-state packet fields coincides with the definition of read/write flanks in Domino \cite{domino}.} The program is then converted into static single-assignment form (SSA)~\cite{ssa} to ensure every variable is written at most once. 

In addition, we perform several static analyses during preprocessing: constant folding, expression simplification, and dead code elimination. These analyses are useful in simplifying the action block of a P4 program, therefore reducing the difficluty of the resultant SKETCH queries. Without these analyses, some functionally-equivalent mutations of our benchmark examples cannot be compiled, as shown later in our evaluation (\S\ref{ssec:codegen-exp}). We neither add or delete stateful variables during preprocessing simplifications, since it is unsound to do so, and we later map stateful variables bijectively to stateful registers in the switch ALUs. SSA-conversion induces more temporary packet fields, some of which are eliminated during preprocessing simplification and later code-generation optimization. The remaining temporaries are treated as metadata in a P4 program.

\begin{figure}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.35\textwidth]{figures/stateful-alu.png}
    \vspace*{-0.1in}
    \caption{Depiction of a stateful ALU. Created during preprocessing of an action block, pre-state packet fields correspond to the pre-state value of ALU registers and post-state packet fields correspond to post-state value of ALU registers.}
    \label{fig:statefulALU}
    \vspace*{-0.2in}
\end{figure}

\subsection{Code Generation Procedure}
\label{ssec:codegen}
We now describe our code generation procedure in detail.
\begin{algorithm}
\DontPrintSemicolon
\SetAlgoLined
\KwIn{Computation graph $G_C = (V, E)$ where $V = V_{stateful} \cup V_{stateless}$.}
\KwOut{Synthesized code for each primary output (PO) and each input to a stateful ALU}
\SetKwFunction{Fmerge}{tryMerge}

\tcp{\scriptsize{Step 1: Normalize the computation graph.}}
Normalize($G_C$); \\
\textbf{assert} \emph{every stateful node in $G_C$ has out-degree 1}\;

\tcp{\scriptsize{Step 2: Perform predecessor packing and folding optimizations.}}
let graphModified := \texttt{FALSE}; \\
\tcp{\scriptsize{Iterate until fixpoint}} 
\While{graphModified} { 
   \tcp{\scriptsize{Folding to eliminate redundant inputs;}}
   \tcp{\scriptsize{returns TRUE iff $G_C$ changed}}
   \For{$(u,v \in E)$, where $v$ is stateful and $u$ is stateless}
     { graphModified := tryFold($G_C$, $u$, $v$)\; }
    \tcp{\scriptsize{Predecessor packing; returns TRUE iff $G_C$ changed}}
   \For{$(u,v) \in E$, where one of $u$, $v$ is stateful}
    { graphModified := tryMerge($G_C$, $u$, $v$)\; }
}

\tcp{\scriptsize{Step 3: Synthesis of stateful updates}}
\For{$v \in V_{stateful}$}
{
success := querySketchStateful(stateVar(v), v)\;
\textbf{assert} success == true\;

}


\tcp{\scriptsize{Step 4: Min-depth synthesis for stateless code}}
O := $POs \cup \{inputs(v) | v \in V_{stateful}\}$\;
\For{$o \in O$}{
%%    \tcp{Find the Backwards Cone of Influence (BCI) of o}
    spec := computeBCI(o) \tcp*{\scriptsize{spec of o}} 
    i := 1 \tcp*{\scriptsize{depth of solution tree}}
    \While{$i \leq $ numPipelinedStages}{
        success := querySketchStateless(o, spec, i)\;
        \If{success == true}{
            \textbf{break} } 
        i++ \tcp*{\scriptsize{increment depth}}
    }
}
%\tcp{Try merging $u$ and $v$ if they fit in a stateful ALU}
%\SetKwProg{Fn}{Function}{:}{}
%\Fn{\Fmerge{$G_c$, $u$, $v$}}{
%    $w$ = union($u$, $v$) \tcp*{combined logic}
%    \If{$\vert inputs(w) \vert$ and $\vert outputs(w) \vert$ meet ALU requirements}{
%        success := querySketchStateful(outputs(w), w)\;
%        \If{success == true}{
%            Replace $u$ and $v$ by $w$ in $G_c$\;
%           Update $V$, $V_{stateful}$, $V_{stateless}$\;
%        }
%    }
%}
\caption{Code Generation Procedure}
\label{alg:1}
\vspace*{-0.1in}
\end{algorithm}

\vspace*{-0.1in}
%\Para{Computation graph construction}
\subsubsection{Computation graph construction}
A dependency graph is constructed from the preprocessed program with nodes for each program statement and an edge for each Read-After-Write (RAW) dependency.\footnote{Conversion to SSA form removes Write-After-Write and Write-After-Read dependencies.} Edges are also added between the pre/post-state packet fields of each state variable. The strongly connected components (SCCs) of this graph correspond to stateful updates, which are condensed to form a \emph{computation graph} $G$. Thus, $G$ is a directed acyclic graph (DAG) with nodes for program computations (some with stateful updates) and edges for RAW dependencies. Nodes in $G$ are partitioned into two sets: \emph{stateful nodes} are formed from SCCs on the dependency graph, containing a set of program statements that describe an atomic stateful update; \emph{stateless nodes} are lifted from the dependency graph and include single program statements operating on packet fields. Each edge $(u, v)$ can be mapped to a packed field variable that represents a LHS (corrsp. output) of $u$ that is a RHS (corrsp. input) in $v$. The sources of $G$ (excluding state variables) are called primary inputs (PIs), i.e., input packet fields that are used in the computation. Inputs to stateful nodes and outputs of sinks of $G$ that are not temporaries (such as pre/post-state packet fields) created during preprocessing are called primary outputs (POs). POs are the final values written to packet fields. 

\subsubsection{Code generation using program synthesis queries}
Given a computation graph $G$, we synthesize code for the POs (packet fields) and state variables such that they are functionally equivalent to the transaction program. The code generation procedure consists of four steps: normalization, predecessor packing and folding optimizations, synthesis of stateful updates, and synthesis of minimum-depth solutions for stateless code. Our code generation procedure is described in Algorithm~\ref{alg:1}.

\begin{figure*}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=\textwidth]{figures/BLUE_DECREASE-opt.pdf}
    \vspace*{-0.1in}
    \caption{Computation graph for BLUE(decrease)~\protect\cite{blue} and sequence of optimizations performed when targeting the Tofino ALU. Stateful nodes shown in blue and stateless nodes in yellow. Pre/post-state packet fields shown in red. Modified lines during optimization shown in bold. }
    \label{fig:normalizeSampling}
    \vspace*{-0.2in}
\end{figure*}

\Para{Step 1: Normalization of computation graph.} We first process the computation graph $G$ in preparation for synthesis of stateful nodes in $G$. The final stateful synthesis step (described in Step 5) will map a stateful node directly to a stateful ALU, which contains at least one stateful register(s) and one output. In the all hardware backends we target (Menshen and Tofino), every stateful ALU is satisfies the following constraint: \emph{a stateful ALU can only output a single value that is either the pre-state or the post-state value of one of its stateful registers}. As such, we cannot directly synthesize any stateful node in $G$ with more than one out edge, as an out edge in the computation graph corresponds to an ALU output. In this step, we normalize $G$ to a graph with out-degree of every stateful node to be at most 1, and such that every packed field labelled in an out-edge from a stateful node is either the \emph{pre-state packet field}, or the \emph{post-state packet field}. An example illustrating the effect of normalization may be found in Figure~\ref{fig:normalizeSampling}.


\emph{Case 1: Handling extra stateful outputs.}
If a stateful node $s\in G$ contains $n > 1$ outputs that are the pre/post-state packet field of a stateful variable, we create exactly $n$ copies of $s_1,...,s_n$ with each copy outputting a distinct output of $s$, delete $s$, and reprocess the graph to add edges that represent input/output dependencies to each newly created node.

\emph{Case 2: Handling extra stateless outputs.}
Otherwise, the stateful node $s$ contains $n$ outputs with $m$ outputs being pre/post-state packet fields of stateful variables and $l$ stateless outputs that are packet fields storing the computation result . Assume there are $k$ stateful registers in a stateful ALU. There are two cases: 
\begin{itemize}
    \item $m<k$. There are $k-m$ scratch registers left; we can use them to compute outputs that depend on pre/post-state packet fields. We again create $n$ copies $s_1,...,s_n$ of $s$ as in Case 1, each $s_i$ a unique output of $s$, delete $s$, and reprocess the graph to add in-/out-edges for the newly created nodes.
    \item $m=k$. There are no scratch registers left. We duplicate the stateful node $2m$ times into $s_1, ..., s_{2m}$ and assign each copy a distinct output that is a pre/post-state packet field in $s$. Next, we build a computation graph $G(s)$ by parsing the read/write dependencies of statements of $s$. For each stateless packet field output $x$ of $s$ that isn't a read or write flank, we add the subgraph $\BCI_{G(s)}(x)$ to $G$. By doing so, we extract stateless output computation out of $s$ into successor nodes whose inputs are the pre/post-state packet fields of stateful variables in $s$, which are provided as outputs of $s_1,...,s_{2m}$. After adding these BCI subgraphs, we delete $s$ and reprocess $G$ to add appropriate input/output dependencies between the newly added nodes.
\end{itemize}

\Para{Step 2: Folding and predecessor packing optimizations.} 
After normalization, we design two optimizations on the computation graph, folding and predecessor packing, that are applied in interleaved fashion until fixpoint. As we later illustrate, the next step of code generation involves mapping each stateful node on the computation graph directly to a stateful ALU in target architecture. Hence we seek to optimize the program such that each stateful ALU \emph{maximally utilizes} the target ALU's capabilities without violating the target ALU's constraints, such as limitations on the number of inputs and outputs.

\emph{Folding to eliminate dependant inputs.} The stateful ALUs in architectures we target have constraints on the max number of inputs and outputs. Since inputs to stateful ALUs directly correspond to inputs to stateful nodes on the computation graph, a stateful node that has too many in-edges could cause the synthesis procedure to fail. The \emph{folding} optimization addresses this issue by finding opportunities to reduce the number of in-edges to a stateful node. Roughly speaking, computations associated with an input to a stateful node can be \emph{folded into} the stateful node if the computations are stateless and the enlarged stateful node can still fit into the target ALU, thereby reducing an input edge. Let $\texttt{inputs}(s)$ denote the set of inputs to a stateful node $s$. A dependant input of $s$ is an input $i\in \texttt{inputs}(s)$ that can be written as the value of a function of other inputs to $s$, i.e. $\texttt{inputs} \setminus \{s\}$. In the folding optimization, we consider stateless dependant inputs to a stateful node $v\in G$. For each such stateless dependant input $i$, we \emph{fold} its associated computation into $v$ and query SKETCH to see if the enlarged stateful node can still be synthesized. If the synthesis query is successful, we eliminate the edge $(u,v)$ where $u$ is the stateless node containing $i$ as a left-hand-side.

To illustrate the folding optimization at work, consider the examples given in Figure~\ref{fig:blue_decrease} and Figure~\ref{fig:dnsTTLExample}, where we compile the BLUE (decrease) and DNS TTL change examples to Tofino and Banzai ALUs, correspondingly. In both examples, the folding optimization helped reduce an edge between a stateless node and a stateful node, thereby reducing the pipeline usage of the compiled program by 1.
  
\emph{Predecessor packing to merge together stateful computations.} Even after folding, the stateful update in a single node in $G$ might not fully utilize the available stateful ALU.  As an example, %if nodes 2 and 3 in 
consider the computation graph for the BLUE (decrease) example in Figure~\ref{fig:blue_decrease}, where there are two consecutive stateful updates.
Here, a single Tofino stateful ALU can actually implement both stateful updates in a single stage. Since pipeline stages are a scarce resource, we would like to reduce the number of stages required by making full use of the switch's ALUs. Hence we would like to attempt \emph{packing} stateful computations in adjacent nodes together, which could reduce the number of stateful ALU usage and thereby potentially reduce the number of used pipeline stages in the compiled program.
%However, the additional functionality of a stateful ALU can be made use of only if the 
%Therefore, we would like to consider multiple nodes in $C$ and possibly merge them if they fit into a stateful ALU. 
%\xiangyu{The Tofino ALU uses one 64-bit register. We consider the first 32-bit as the first stateful var and the second 32-bit as the second stateful var. I am not sure whether we can mention this details in the paper without violating NDA}

More generally, optimal code generation for a DAG 
%(i.e., for language expressions with common subexpressions) 
is known to be NP-complete~\cite{AJU77}. 
%This problem is also similar to the problem of technology mapping in hardware design, and a practical approach is to partition the DAG into a forest of trees, and solve each tree problem optimally using dynamic programming~\cite{KeutzerDac87}. 
%would require considering all possibilities which would be infeasible for large graphs. Instead, we use a greedy strategy shown in Algorithm~\ref{alg:1}, lines 5 to 11. In reverse topological order, we traverse pairs of adjacent nodes (we ignore nodes with no dependencies as they can be scheduled in parallel) with at least one stateful node, 
Here, we use a simple heuristic for optimization, called \emph{predecessor packing}, inspired by similar work in technology mapping for hardware designs~\cite{flowmap}. The main idea is to pack more into a stateful ALU by possibly merging pairs of nodes $u$ and $v$, at least one of which is stateful.
% at node $v$, by possibly merging it with its predecessor node $u$ (which could also be stateful). 
To avoid lengthening other paths in $G$, we only consider a predecessor $u$ that has no other fanouts. 
This is implemented in the function $tryMerge$, which first uses an inexpensive check on the number of inputs and outputs in the combined logic for $u$ and $v$, and then calls a SKETCH synthesis query to check if both can fit into a single stateful ALU.
If the query is successful, we merge the two nodes in $G$.

\emph{Optimizing the computation graph by iteratively folding and packing.} We iteratively apply folding and predecessor packing on the computation graph $G_C$ until fixpoint, terminating when the optimizations make no further modifications to the computation graph. Iteratively performing folding guarantees that after convergence, no stateful nodes contain dependant inputs that can be eliminated. Iteratively performing predecessor packing guarantees that after convergence, each stateful update in $G$ is \emph{locally maximal} in the sense that it cannot be merged with any predecessor node (with no other fanouts)
and still fit within a stateful ALU. We show the effectiveness of this optimization in our evaluation (\S\ref{ssec:codegen-exp}), where its use results in fewer stages in the solution. 

\begin{figure}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.4\textwidth]{figures/Sampling-Normalized-UPDOWN.pdf}
    \vspace*{-0.1in}
    \caption{Pre- (top) and post-normalization (down) comparison of the computation graph for the Sampling benchmark program. Stateful nodes are in blue and stateless nodes are in yellow. Newly added succcessor nodes during normalization are colored in orange. }
    \label{fig:normalizeSampling}
    \vspace*{-0.05in}
\end{figure}

\begin{figure}
    \centering
    \vspace*{-0.1in}
    \includegraphics[width=0.5\textwidth]{figures/DNS_TTL_1-new.pdf}
    \vspace*{-0.1in}
    \caption{A subgraph of the DNS\_TTL\_Change benchmark example before (left) and after (right) folding, when compiling to the Banzai ALU with the FPGA backend. Note the folding optimization reduced an edge (corresp. an input). Stateful nodes shown in blue and stateless nodes in yellow. Pre/post-state packet fields shown in red. Modified lines during optimization shown in bold.}
    \label{fig:dnsTTLExample}
    \vspace*{-0.2in}
\end{figure}


\begin{figure}
    \centering
    \includegraphics[width=0.51\textwidth]{figures/Computation-Graph-labelled.pdf}
    \caption{Example of a computation graph with a single stateful node (4) and its code generation result targeting Banzai ALU. Stateful nodes are in blue and stateless nodes are in yellow. The POs are $\textsf{p.o1,p.o3}$. The BCI of $\textsf{p.o1}$ contains nodes 1, 2 and the BCI of $\textsf{p.o3}$ contains nodes 1, 3.  } 
    \vspace*{-0.2in}
    \label{fig:codegen_example}
    % \hfill
    % \begin{subfigure}{0.5\textwidth}
    % \includegraphics[width=\textwidth]{hotnets21-template/Figures/codegen_soln.png}
    % \caption{Synthesized solution.}
    % \label{fig:codegen_example_soln}
    % \end{subfigure}
    % \caption{Example computation graph and synthesized code.}
\end{figure}


\Para{Step 3: Synthesizing stateful updates.} 
First, we consider the stateful updates in $G$. To preserve the packet transaction semantics of the program, each stateful update must be completed in a single pipeline stage, so that the computation finishes by the time the next packet arrives. Thus, it \emph{must} fit within a single stateful ALU, since state cannot be shared across ALUs. For each stateful node in $G$, we generate a SKETCH query to check if the stateful update can be implemented by a stateful ALU, modeled using a SKETCH grammar $A_1$, and assert that the query succeeds. If a query fails, our procedure terminates with an error. 

% \vspace*{-0.1in}
\Para{Step 4: Minimum-depth solutions for stateless code.} 
After the first two steps, all stateful nodes in $G$ are mapped to stateful ALUs and are locally maximal. We now need to synthesize code for the inputs to these stateful ALUs and the POs of $G$. 
For each variable $o$ to be synthesized, we first compute 
%its specification in terms of PIs and outputs of stateful ALUs (at the end of step 2), by computing 
its backwards cone of influence (denoted as $\BCI_G(o)$), which is often used in verification/synthesis tasks to determine the dependency region (up to some boundary)~\cite{SomenziBook}. In graph-theoretic terms, $\BCI_G(o)$ is a subgraph in $G$ derived by going recursively backward from $o$, stopping at a PI or a stateful node. Essentially, $\BCI_G(o)$ provides the \emph{functional specification} for $o$ in terms of PIs and outputs of stateful ALUs in $G$. Note that these specifications are stateless since they do not include any stateful nodes. 

We model the switch's stateless ALU functionality also using a grammar, say $A_2$, and then use SKETCH to find a \emph{minimum-depth tree} solution for $o$, where each tree node denotes a stateless ALU allowed by the grammar $A_2$. Since SKETCH cannot directly optimize for minimum depth, we invoke SKETCH in a loop, to find a solution tree of a given depth $i$, %(line 17), 
and iteratively increment $i$ starting from 1. We stop as soon as a solution is found, or if $i$ exceeds the maximum number of pipeline stages. 
%Thus, this step returns a solution tree with the minimum number of pipeline stages. 

% \aarti{maybe we can show only one of the outputs, and put the two figures into one? or skip entirely?} 
% \ngs{I would support showing one output and merging figures given that space is an issue.}
An example computation graph with two stateful updates (gray boxes) and the synthesized solution for one of them is shown in Figure~\ref{fig:codegen_example}; the solution for the second is similar. The stateless updates for $p.o2$ and $p.o3$ need three stages using our algorithm; converting to three-address code, as Domino does, would have required four stages. 
%Although the depth of a solution for each synthesized variable is guaranteed to be minimum, the overall solution might have a larger \emph{width} than required. 
%In our example, 
%in Figure~\ref{fig:codegen_example_soln} 
%note that the updates 
%Although $p.o2$ and $p.o3$ share the update to $p.o1$ (node 1); however, the synthesized solution 
%might not have shared code 
%does not, since separate Sketch queries are used for outputs $p.o2$ and $p.o3$. We leave the synthesis of solutions \emph{with sharing} to future work.
% We leverage min-depth tree algorithm to do code generation for each action portion. At a really high level, the goal of using min-depth tree is to generate code with minimum number of stages for one given program. The whole algorithm can be divided into several stages. The first three stages, which aims at building dependency graph after parsing the input program, are similar to what Domino compiler has done. However, since naively using the dependency graph generated from the first three steps might be unnecessarily large in terms of the depth of that tree, in order to make the tree more compact, the remaining steps are implemented in sequence. Based on the generated dependency graph, step 4 tries to separate SCCs from WCCs since we will use different procedures for code generation. As for SCCs, a single SKETCH is used to check whether a stateful ALU can implement the stateful update or not, while as for other WCCs, we treat each component as the specification and a grammar, which captures the switch functionality and is parameterized by an integral bound, is considered as implementation. Given a bound of depth, SKETCH is used to check whether there exists an implementation that can fully express the given input program. Since the bound starts from one and we increment the bound by one each time, this procedure is capable of finding the expression tree of minimum depth that satisfies the specification. With the generated code in hand, step 6 combines the results from SCCs and WCCs by preserving their dependency relationships. Finally, the last step, optimization step, checks the possibility of merging adjacent nodes of stateful super nodes to eliminate more components by fully utilizing the additionaly functionality from stateful ALU on top of the stateful updates. The final optimization step offers a second chance to reduce the total number of depth of our generated code.

\subsubsection{Correctness and Optimality of Code Generation}

\ruijie{We need to rewrite this section; it attracted bad feedback from NSDI reviewers.} 
The final result of all three steps in code generation is in the form of a resource graph $R$, where each node $v$ is mapped to either a stateful or a stateless ALU, and an edge $(u, v)$ indicates that an output of the ALU at $u$ is connected to an input of the ALU at $v$. 
%The PIs, POs, and state variables in $R$ are the same as in $C$. 
Due to the guaranteed correctness of program synthesis in SKETCH over a bounded input range, the POs and stateful updates in $R$ are guaranteed to be functionally equivalent to those in $G$ for the same input range. The predecessor packing in Step 2 results in locally maximal use of stateful ALUs, and the min-depth tree solutions in Step 3 are optimal in using a minimum number of stages with stateless ALUs. Note also that each SKETCH query in our procedure is smaller than a query for the full transaction, thereby resulting in significant performance improvement overall, as demonstrated later in our evaluation (\S\ref{sec:eval}).

%In terms of comparison, the Chipmunk compiler~\cite{chipmunk} also supports transactions, but it invokes program synthesis on an \emph{entire transaction scope} in an individual synthesis query, which leads to long and variable synthesis times, even with a slicing-based technique.
%that creates smaller subproblems for synthesis. 
%In contrast, our approach separates the synthesis of stateful updates from stateless updates, since the former are critical for successful code generation, and the latter queries are over possibly smaller subgraphs that comprise stateless logic regions between stateful updates\footnote{This is inspired in part by logic synthesis in hardware design~\cite{SomenziBook}, which optimizes  combinational logic between stateful updates.}. 
%As shown later in our evaluation (\S\ref{sec:eval}), our compiler achieves 
%the same minimum number of pipeline stages 
%comparable quality of results as Chipmunk, but with significant speedup in runtimes. 
%Another big difference is that Chipmunk does not consider multiple transactions or pack them in the pipeline stages.

\subsection{Constraint-based Resource Allocator}
\label{ssec:resource_allocation}

The second phase of our compiler uses a
%integer linear programming (ILP) 
constraint-based formulation
to allocate resources such as 
memory blocks and ALUs for P4 language constructs such as tables and expressions.
% , and registers. 
The constraints for memory blocks are similar to prior work by Jose et al.~\cite{lavanya_nsdi15}. In addition to Jose et al.'s formulation, we formulate constraints for ALUs.
% and table resources.
%One distinctive feature of our formulation is that 
We aim to allocate resources for \emph{multiple actions} in each pipeline stage 
as long as the corresponding computations have no dependencies, which we identify from a table dependency graph (similar to prior work~\cite{lavanya_nsdi15,cetus}). Moreover, unlike prior work~\cite{lavanya_nsdi15,cetus}, our formulation can handle multi-stage actions as well as atomic transactions. 
We use the resource graph $R$ derived for each action (after code generation) to enforce {\em intra-table constraints}, and use the table dependency graph to enforce {\em inter-table constraints}. In the remainder of this section, we describe our resource allocation constraints with reference to a generic RMT design; these can be easily extended to other hardware resources in a specific architecture.
%Our formulation extends Jose et al.'s formulation~\cite{lavanya_nsdi15} with constraints over ALUs.

\Para{Constants.} We use the following constants:
%in our formulation:
%to represent maximum limits on hardware resources: 
\begin{CompactItemize}
    \item 
$N_S$ denotes the maximum number of pipeline stages.       \item 
$N_{alu}$ denotes the maximum number of ALUs in each stage (could be generalized to be different per stage).
    \item 
$N_{table}$ denotes the maximum number of logical table IDs per stage.
    \item 
$N_{entries}$ denotes the maximum number of match entries per table in each stage.
    \item 
For table $t$, we use a constant $e_t$ to denote the %maximum% 
number of match entries in the table, as specified in the program.
\end{CompactItemize}

\Para{Handling tables with too many entries.} If a table $t$ has too many entries ($e_t > N_{entries}$) to fit within a single stage, we partition these entries into $b_t$ separate tables that can each fit within a single stage, where $b_t = \lceil(e_t/N_{entries})\rceil$. If the match type is exact, a packet will match at most one of these $b_t$ tables, and they can be regarded as independent tables with the same actions as table $t$. Our partitioning procedure could be extended in the future to support other types of matches.

\Para{Handling multi-stage actions.} We handle a multi-stage action under the condition that it 
%Assuming that a multi-stage action 
does not modify the table's match key, by duplicating the match entries at each stage to ensure that the entire action is executed. For example, suppose match entry $m$ in table $t$ is associated with action $A$ that takes 2 stages, $s_1$ and $s_1 + 1$. We allocate table $t$ in both stages $s_1$ and $s_1 + 1$. If a packet matches entry $m$ in table $t$ in stage $s_1$, it will match entry $m$ in table $t$ in stage $s_1 + 1$ as well, resulting in action $A$ being executed completely. 
If Action $A$ is allocated to non-consecutive stages, we allocate additional ALUs in the intermediate stages
%duplicate the match entries in each intermediate stage\xiangyu{Actually, we do not duplicate the match entries in all intermediate stages. We only duplicate in stages that ALUs belonging to that action appear}, using ALUs (\hl{AG: this seems specific to FPGAs, should we mention that other PISA architectures could use PHVs?}) 
to propagate the intermediate results to the next stage. Note that Menshen requires additional ALUs for propagation of intermediate results; other RMT architectures could use, for example, dedicated ``tag-along'' PHV containers for propagating intermediate results. Thus, propagation constraints apply to either ALUs or to PHV container resources, depending on the specific architecture. Note that with PHVs, these constraints would allow sharing of PHVs for variables with different lifetimes.

\Para{Variables.} 
% integer variables $S_t$ and $E_t$ denoting the starting and ending stages allocated to the table (as a design decision, we choose to allocate each table in consecutive stages), and
% an integer variable $M_{ts}$ denoting the number of memory units in stage $s$ allocated to the table.
For the $a^{th}$ action in the $i^{th}$ partition of table $t$, we use $R_{tia} = (V_{tia}, E_{tia})$ to denote the corresponding resource graph which is computed in the code generation phase. Recall that this resource graph could span multiple stages. For each partition $i$ of table $t$, we use a binary variable $M_{tis}$ which is $1$ if the match part of the table is assigned to stage $s$, and $0$ otherwise. We use an integer variable $stage_{u}$ to denote the stage assigned to ALU $u$, and a corresponding binary variable $stage_{us}$ which is $1$ if ALU $u$ is assigned to stage $s$ and $0$ otherwise.

We define $I$ to be the set of ALUs whose outputs are intermediate variables (i.e., temporary packet fields or pre/post-state packet fields of state variables), and $R_u$ to be the set of ALUs that read the output of ALU $u$. These sets are computed by analyzing the resource graph of each action. For each ALU $u$ in $I$, we use an integer variable $beg_u$ to denote the stage the computation is performed and an integer variable $end_u$ which is at least as large as the last stage where the output of ALU $u$ is used. For each ALU $u \in I$, we use a binary variable $prop_{us}$ which is $1$ if an additional ALU that propagates the result of ALU $u$ to the next stage is assigned to stage $s$, else $0$.


\Para{Constraints.}
We now describe the constraints in our formulation. We begin with constraints related to allocation of table entries, and dependencies between tables. These extend the formulation in prior work~\cite{lavanya_nsdi15} by dealing with actions, where actions can possibly span multiple stages. 
% (similar to prior work~\cite{lavanya_nsdi15}). 
%except we abstract away some details of memory allocation.

%\noindent
% \paragraph{Memory allocation constraints.}  For each table, the total number of memory units allocated must be at least as large as the number of table entries.
% \begin{equation*}
%     \sum_s M_{ts} \geq e_t 
% \end{equation*}

\Para{Match constraints.} For every ALU assigned to a stage, its corresponding match entries must also be assigned to that stage.
\begin{equation*}
    \forall s \ \forall t, i, a \ \forall u \in V_{tia}: \ \ \ stage_{us} = 1 \rightarrow M_{tis} = 1
\end{equation*}

\noindent
\Para{Table dependency constraints.}
We consider four types of table dependencies: match, action, successor, and reverse-match~\cite{lavanya_nsdi15}.
If table $t_2$ depends on table $t_1$, all ALUs of $t_2$ are allocated after ALUs of $t1$. For successor and reverse-match $<$ below should be replaced by $\leq$.
\begin{align*}
    & \forall i_1, i_2, a_1, a_2, \forall u_1 \in V_{t_1\ i_1\ a_1}, \ \forall u_2 \in V_{t_2\ i_2\ a_2}: \\
    & stage_{u_1} < stage_{u_2}
\end{align*}
%\hl{AG: do we need forall u2 in above?}\xiangyu{Yes, we do need forall since we only care about action level dependency rather than ALU level dependency. Based on our constraints, if it is match/action dependency, it is $stage_{u1} < stage_{u2}$ while as for successor/reverse dependency, it should be $stage_{u1} \leq stage_{u2}$}

\noindent
\Para{Action dependency constraints.} The allocation of ALUs to stages must respect the dependencies within an action, given by the edges of the corresponding resource graph $R_{tia}$. If the output of ALU $u$ is an input of ALU $v$, then $u$ must be allocated in an earlier stage than $v$.
\begin{equation*}
    \forall t, i, a \ \forall (u, v) \in E_{tia}: \ \  stage_u < stage_v
\end{equation*}

\noindent
\Para{Propagation constraints.} If ALU $v$ depends on ALU $u$ and they are not allocated in consecutive stages, we allocate additional ALUs to propagate the output of ALU $u$ until the stage assigned to ALU $v$.
% \hl{AG: using an ALU for propagation seems specific to the FPGA, should we note that PHV containers could be used in other architectures?}

The output of $u$ is computed in $stage_u$, and $beg_u$ must be less than $end_u$.
\begin{align*}
   &\forall u \in I: \ \ beg_u = stage_u\\
   &\forall u \in I: \ \ beg_u < end_u
\end{align*}
Variable $end_u$ must be as large as the stage assigned to any ALU $v \in R_u$ that uses the result of ALU $u$.
\begin{align*}
    &\forall u \in I, \forall v \in R_u: \ \ end_u \geq stage_v\\
    &\forall u \in I: \ \ end_u \leq N_S
\end{align*}
For all stages $s$ where $beg_u < s < end_u$, we must allocate an ALU to write the output of $u$ to the next stage.
\begin{equation*}
    \forall u \in I, \forall s \in \{1,\ldots,N_S\}: \ \ (beg_u < s \land s < end_u) \leftrightarrow prop_{us} = 1
\end{equation*}
If an ILP solver is used, the above constraints can be formulated using the well-known Big-M method, as shown in Appendix~\ref{appendix:bigm_encoding}.

\noindent
\Para{Resource constraints.}
The stage allocated to each ALU must be within the range of available stages.
\begin{equation*}
    \forall t, i, a \ \forall u \in V_{tia}: \ \ 1 \leq stage_{u} \leq N_S\\
\end{equation*}
The number of ALUs allocated in each stage must be less than or equal to the number of ALUs available, $N_{alu}$. We allocate $H$ ALUs per stage to transport the packet header fields through the pipeline. We need to make sure that the number of ALUs for intermediate fields
%\xiangyu{and stateful variables. (Because stateful ALUs also need allocation)} 
is no more than $N_{alu} - H$.
Note again, that the $H$ constraint is specific to our FPGA platform that uses ALUs for propagation (as described earlier); other architectures need not use ALUs for propagation. 
%\hl{AG: again, isn't this specific to the FPGA?}\xiangyu{This should be substrate-specific to this FPGA design}
\begin{align*}
&\forall s\ \forall t, i, a,\ \forall u \in V_{tia}:\ \  stage_{u} = s \leftrightarrow stage_{us} = 1\\
&\forall s\ \forall u \in I: \ \  stage_{us} + prop_{us} \leq N_{alu} - H
\end{align*}
Finally, the number of tables allocated in a stage must be less than or equal to the number of table IDs available, $N_{table}$.
\begin{equation*}
    % \forall s \in \{1, \ldots, N_S\} \sum_{t, i} I(\bigvee_{u \in V_{ti}} stage_u == s) \leq N_{table}
    \forall s: \ \ \sum_{t, i} \ \ M_{tis} \leq N_{table}
\end{equation*}

\noindent
\Para{Solving the constraint problem.}
We can use either an ILP solver (Gurobi~\cite{gurobi}) or an SMT solver (Z3~\cite{z3}) to find either an optimal or a feasible solution, depending on the choice made by a user. (Note that Z3 supports optimization with the theory of linear integer arithmetic.)
 %\xiangyu{In the ILP file, we allow users to set the mode flag. The default mode is optimization while if they set it to feasibility on purpose, the ILP solver will output one feasible solution.}
%\noindent
%\paragraph{Optimality constraints.} 
\begin{itemize}
    \item Optimality constraint: 
If the user chooses to find an optimal solution, they can optionally specify an objective function. For example, one can minimize the number of stages occupied, since this is often the most scarce resource within a switch. Formally, the objective function is $\min\ cost$ where $cost$ is greater than or equal to the stage assigned to every ALU: $\forall t, i, a,\ \forall u \in V_{tia}:\ cost \geq stage_u$.

% \hl{AG: please add a small para on finding a feasible solution below.}
%\noindent
%\paragraph{Feasibility constraint.}
\item Feasibility constraint: 
If the user opts to find a feasible (but not necessarily an optimal) solution, we use a trivial objective function such as $min\ 1$ with Gurobi. With Z3, we omit an optimization function, and simply let it find a feasible solution.
\end{itemize}
%\hl{AG: Instead of above para on Feasible solution, add a para on "Solving the Constraint Formula" and describe how we can use either Gurobi or Z3 to find either an optimal or a feasible solution.}\xiangyu{In the ILP file, we allow users to set the mode flag. The default mode is optimization while if they set it to feasibility on purpose, the ILP solver will output one feasible solution.}

\iffalse
The result of the code generation phase is a resource graph for each action in the P4 program. We denote the resource graph for the $i^{th}$ action in table $t$ by $R_{ti}$. The resource graphs of non-atomic actions consist of a single node representing the ALU which implements the update. %\aarti{please explain -- is such an action a single update? We would have checked that it fits, right?}
Due to space limitations, we describe allocation of ALUs from resource graphs for actions; handling memory blocks is similar to prior work~\cite{lavanya_nsdi15}.

Given these resource graphs, one for each P4 action, the second phase of our compiler uses an ILP to pack the resource graphs into the switch's pipeline stages so that they take the minimum number of stages, while respecting the dependencies %between nodes 
in each resource graph as well as the dependencies between tables. The objective function of the ILP minimizes the total number of stages, and the constraints encode the resource constraints of the switch and the dependencies between resources. 
% We specify the objective function and describe how to encode chip-specific constraints for our ILP scheduler based on our best-effort understanding of the Tofino switch. These constraints are the key determinant for our final ILP optimization problem. 
\iffalse %%AG moving this to later, after the constraints
\Para{Objective function} We use an objective function that minimizes the total number of stages occupied since this is the most scarce resource within a switch. Formally, the objective function is $\min cost$
% where for all tables $t$ and all ALUs $i$, $cost \geq t\_Act\_i$ where $t\_Act\_i$ is the stage assigned to the ith ALU of table $t$.
where for all tables $t$, all actions $i$, and all nodes $u \in R_{ti}$, $\ cost \geq stage_u$, with $stage_u$ denoting the stage number assigned to node $u$.
% Why does optimization matter (relative to satisfiability) on all-or-nothing line rate?
\fi %%AG end of iffalse
%\paragraph{ILP Constraints}
%\subsubsection{ILP Constraints} 
There are two main types of constraints in our ILP formulation: resource constraints and dependency constraints.
%\aarti{what about memory block constraints -- we should say something even if our benchmarks didn't use any.}

\noindent
\textbf{Resource constraints.} For each ALU $u$ in each resource graph, we define 
% $n$ as the total number of ALUs required for its actions and
$stage_u$ as the stage number allocated to it. We define $N_{alu}$ as the total number of ALUs available per stage and $N_{table}$ as the total number of logical table IDs per stage. The resource constraints are encoded below, where $I(c)$ is an indicator variable that is equal to $1$ if condition $c$ is true and $0$ otherwise.\\
$\forall s, \sum_{t, i} \sum_{u \in R_{ti}} I(stage_u == s) \leq N_{alu}$.\\
% $\forall s, \sum_{t, i} I(t\_Act\_i == s) \leq N_{table}$.\\
%$\forall s, \sum_{t, i} \sum_{u \in R_{ti}} I(stage_u == s) \leq N_{table}$.\\
$\forall s, \sum_{t, i} I(\bigvee_{u \in R_{ti}} (stage_u == s)) \leq N_{table}$.\\
%\todo{check: isn't this counting each action in each table?}
%\aarti{please explain what is denoted by I(.). The second constraint doesn't seem correct -- if two ALUs from action of the same table are assigned to stage s, this should still be counted as only 1 table -- you should not sum over ALUs from the same table for checking against N\_table}
%\xg{Hi Aarti, this is an issue of our current setting. When we divide one atomic action block into multiple ALUs, we need to put each ALU into one new table so as to implement its functionality. Therefore, we need to sum over ALUs from the same table. But maybe we need to clarify this point to avoid any misunderstanding.}
%\ngs{I too got tripped up by the second constraint above, like the others seem to have. }

\noindent
\textbf{Dependency constraints.} 
In addition, the solution must respect the dependencies between logical tables (inter-table dependencies) and within each logical table (intra-table dependencies). 
If table $t_{2}$ depends on table $t_{1}$, then any ALU of $t_{2}$ is allocated \emph{after} any ALU of $t_{1}$, using the following constraint:
%To be specific, if table $t_{2}$ depends on table $t_{1}$, then any ALU of $t_{2}$ should be allocated \emph{after} any ALU of $t_{1}$: \ngs{Should it? It depends on which ALU induced the table-level dependency, no? May rephrase as ``we use the following constraint to allocate any ALU of t2 after any ALU of t1''}\\
% if $t_{2}$ depends on $t_{1}$, $\forall i, j, t_{1}\_Act\_i \leq t_{2}\_Act\_j$.\\
$\forall i, j \ \forall u1 \in R_{t1i}, u2 \in R_{t2j}, \   stage_{u1} < stage_{u2}$.\\
The intra-table dependencies are given by the edges of the resource graph for each action in a table.
% As for all ALUs generated for action in a specific table $t$, in order to preserve the semantics, the resource allocation for them must be consistent with the order from code generator.
% If $t\_Act\_i$'s output is an input of $t\_Act\_j$, then we must allocate $t\_Act\_i$ to in an earlier stage than $t\_Act\_j$:\\
% for table $t$, if $ALU_{j}$ depends on $ALU_{i}$, $t\_Act\_i \leq t\_Act\_j$
If node $u$'s output is an input of node $v$, then $u$ must be allocated to an earlier stage than $v$.
For each resource graph $R_{ti} = (V_{ti}, E_{ti})$,
$\forall (u, v) \in E_{ti}, stage_u < stage_v$.
% ILP technique used to encode various constraints
% Constraint 1: # of available ALUs per stage
% Constraint 2: # of available tables per stage
% Constraint 3: inter-table dependency (table level dependency)
% Constraint 4: intra-table dependency (action level dependency)

%\paragraph{Objective function}
%\subsubsection{ILP Objective Function}
\noindent
\textbf{ILP Objective Function.}
We use an objective function that minimizes the total number of stages occupied since this is the most scarce resource within a switch. Formally, the objective function is $\min cost$
% where for all tables $t$ and all ALUs $i$, $cost \geq t\_Act\_i$ where $t\_Act\_i$ is the stage assigned to the ith ALU of table $t$.
where for all tables $t$, all actions $i$, and all nodes $u \in R_{ti}$, $\ cost \geq stage_u$.
% with $stage_u$ denoting the stage number assigned to node $u$. (defined previously).
% Why does optimization matter (relative to satisfiability) on all-or-nothing line rate?

\fi 

%\subsection{Combination of both generator and allocator}
%\subsection{CaT Compiler Workflow}

==> intro_asplos23.tex <==
\section{Introduction}

High-speed and programmable packet-processing pipelines are emerging as important programmable platforms. Examples of such platforms include the Tofino~\cite{tofino}, Trident, and Jericho switches and the Pensando and Intel IPU network-interface cards (NICs). Concurrently, P4 is emerging as a popular language to program such platforms.

Compiling P4 programs to these pipelines is a challenging compiler problem. At its core, the compiler's task is to solve a hard combinatorial optimization problem to ``pack'' the P4 program's computations into the pipeline's resources. This combinatorial optimization problem has several distinguishing features that make solving the problem challenging. One, it involves multiple resources such as memory blocks, computation units, and crossbars. Two, a P4 program's computations must be transformed into configurations for computation units such that the computation units faithfully implement the semantics of the P4 program. Three, resources can sometimes be used interchangeably to realize the same computation, e.g., using a lookup table in place of a large number of if-else branches. Four, dependencies between computations can leave some resources unused even if these resources could be used for some computations.\xiangyu{Point no.4 is a little bit confusing. Not sure what does it mean?} And five, some resources may have to be allocated together, e.g., memory blocks and action units within a match-action table.\xiangyu{should we stick to use either lookup table or match-action table across the paper?}

Prior projects have tackled several individual aspects of this compilation problem. Domino~\cite{domino} and Chipmunk~\cite{chipmunk} deal with the code generation problem of mapping a transactional specification of packet processing to computation (action) units in the underlying hardware. Lyra~\cite{lyra} and Jose et al.~\cite{lavanya_nsdi15} deal with the resource allocation problem of allocating computations to resources present in the underlying hardware. Cetus~\cite{cetus} rewrites P4 programs that cannot be compiled (by a commercial compiler) into semantically equivalent versions of the same P4 program that can actually be compiled.
% TODO: Say something about Lucid and P4All here.

In this paper, we present an end-to-end compiler, \sysname, that unifies these prior approaches and translates high-level P4 programs into a low-level representation suitable for hardware execution. Our main idea is to adapt high-level synthesis (HLS)---a technology for productive and high-performance hardware design for ASICs~\cite{hls_asic} and FPGAs~\cite{hls_fpga}---to the new domain of packet pipelines.

HLS~\cite{hls} is an approach to digital design that aims to improve designer productivity while still providing high performance of the resulting design. Informally, HLS takes as input a high-level algorithmic description of the hardware design with no reference to clocks or pipelining, and with limited parallelism in the description. A HLS compiler then progressively lowers this high-level description down to a low-level and optimized implementation: pipelining the implementation if possible, executing multiple computations in parallel, and mapping computations down to a register-transfer level (RTL) design with clocked registers. HLS has been applied to the design of ASICs~\cite{hls_asic} and FPGAs~\cite{hls_fpga}. In this paper, we adapt the idea of HLS to the domain of high-speed packet processing pipelines---an emerging and important compiler target.

Our HLS\xiangyu{Maybe we should say "our CaT compiler" rather than "our HLS compiler"} compiler consists of three phases that roughly mirror a traditional HLS compiler, but are adapted to the new domain of packet pipelines. The first phase employs \emph{resource transformations} that rewrite a high-level P4 program to another\xiangyu{semantically equivalent but syntactically different} high-level P4 program; these rewrites are used to transform a computation's use of one resource (which is scarce) to its use of a different resource (which is relatively abundant)\doris{can we just say "of one scarce resource to its use of another relatively abundant resource"}. The second phase implements \emph{resource synthesis} to lower transactional blocks of statements in the high-level P4 program to a lower-level version of P4. In this lower-level version of P4, individual computation and accelerator units are synthesized to realize the programmers' intent in the transactional blocks, while respecting the computational constraints of these units. The third phase performs \emph{resource allocation} to allocate blocks in the lowered P4 program to physical resources (such as ALUs and memory blocks) on the chip.

Each of these phases uses different techniques, but utilize a common intermediate representation (IR) inspired by RMT~\cite{rmt}. \doris{I think this is the first time RMT shows up in the main body, should we use the full name?} Specifically, our normalized IR is based on match/action table processing, where each action is a high-level (possibly complex multi-stage) transactional block. Resource transformations work on the abstract syntax tree (AST) of the P4 program, visiting various AST nodes to transform them into other AST nodes that represent an equivalent P4 program. Resource synthesis is employed on each transactional block in the IR. It uses program synthesis techniques, specifically the SKETCH~\cite{sketch} syntax-guided synthesis engine, where the transactional block serves as the specification and the implementation is synthesized from a grammar that describes the space of computations permitted by each computational unit available in the target. Resource allocation is then used to pack all transactional blocks in the IR into available hardware. It uses constraint satisfaction solvers, in the form of the Gurobi~\cite{gurobi} ILP and Z3~\cite{z3} SMT engines, to assign low-level P4 blocks to physical resources on the chip, by finding either a feasible or an optimal solution\xiangyu{an optimal or a feasible solution. (map to Gurobi ILP and Z3 SMT)}. Crucially, these phases allow us to take an input program written in P4 and transform it into a low-level representation for hardware execution, without requiring the programmer to develop programs in a new language, in contrast to some prior approaches~\cite{domino, chipmunk, lyra, lucid, p4all}.
% Point to make: You can use higher level languages like Lucid and Lyra to compile down to P4.
% Our goal is to provide a narrow-waist compiler for P4 down to the final hardware target.

The main benefit of our three-phase approach is that it modularizes the overall combinatorial optimization problem into smaller tasks, while still enabling a high-quality result. In addition, we improve upon the state of the art and introduce new techniques in each phase. In particular, our resource transformations are powered by a novel \emph{guarded dependency analysis} in P4 programs to identify opportunities for transforming certain conditional statements in the control block into match/action tables that use less scarce resources. Our resource synthesis phase uses a novel synthesis procedure that uses SKETCH~\cite{sketch} on small subproblems to find a solution that has locally minimal \emph{depth}, i.e., number of pipeline stages, which is often a critical resource in RMT~\cite{rmt} switch hardware. Finally, our resource allocation phase builds on top of prior work by Jose et al.~\cite{lavanya_nsdi15} and extends it to handle complex actions (via results of our resource synthesis phase) and multiple transactions in P4 programs, and a more detailed formulation of the hardware constraints of a cycle-accurate simulator of an RMT pipeline~\cite{menshen}.\xiangyu{should we mention Tofino in addition to a cycle-accurate simulator here?}

We prototyped these ideas by designing a compiler, \sysname, that follows our proposed HLS workflow for programmable packet-processing pipelines in the style of RMT. To effectively evaluate \sysname we need a hardware target that supports fine-grained resource allocation and control over the configuration of computation units. Unfortunately, existing commercial switch pipelines have proprietary instruction sets and do not support the kind of low-level access required to prototype \sysname. Hence, we extended Menshen~\cite{menshen_site}, an open-source register-transfer level (RTL) Verilog model of an RMT pipeline, to serve as a hardware target. Because it is written in RTL, this target supports cycle-accurate simulations and can eventually be synthesized into an FPGA or ASIC prototype, although we have not yet performed this synthesis.\xiangyu{Can we say sth. like synthesis is beyond the scope of this paper rather than raise a potential point for reviewers to complain. Why not perform synthesis?} We also built a partial backend for the Tofino~\cite{tofino} programmable switch by generating low-level P4 in lieu of machine code.\xiangyu{Can we first mention building a partial backend and then say we target cycle-accurate simulations? It makes more sense to me since that is the motivation for us to consider cycle-accurate simulator as another backend.}
% We think this could be a blueprint for how such compilers can be built going forward.

% Chipmunk was trying to solve: rewrite, codegen, and resource allocation all in one shot, which is why it needed so much compilation time, and was restricted to a single transaction. Chipmunk is one piece of evidence that doing it in a monolithic fashion is too hard.

==> intro_nsdi22.tex <==
\section{Introduction}
Programmable packet processing has come of age with several high-speed programmable devices---both switches and network interface cards (NICs)---now commercially available. Concurrently, programming languages with broad community support such as P4 and NPL have emerged as a way to ease the programming of these devices. Yet, programming these devices still remains challenging for two primary reasons. First, the computational units on these devices permit only a restricted set of packet transformations to ensure they can maintain line rate. Second, the number of these computational units and amount of memory available on these devices is limited.

%\hl{AG: A recent} work~\cite{cetus} has proposed merging tables in a P4 program to enable fitting the program within the given hardware resources. Such program-level transformations are complementary to our approach.\xiangyu{Should we add one sentence to briefly describe our approach? e.g. complementary to our approach, which tries to fit the program into hardware using the least amount of resources.}
%By contrast, we believe that both the languages and devices themselves are adequate for their intended use cases, as demonstrated by the many creative uses of programmable networks~\cite{netcache, netchain, netpaxos, switchml, xenic}. Instead, we contend that the problem lies with the compiler that bridges the gap between the language and the device.
Several prior research efforts have observed this state of affairs and have proposed new hardware architectures~\cite{drmt, stateless_quo} and programming languages~\cite{lyra, lucid, p4all} as remedies. Even with these advancements on the language and hardware fronts, the core problem remains that a compiler must bridge the ``last-mile'' gap from some low-level program representation to resource-constrained hardware. The focus in our paper is on this compiler.

An ideal compiler to hardware should be able to handle the fact that (1) there are restrictions on packet transformations at line rate and (2) only a limited number of resources are available, and yet still compile a program to the underlying device---if it is theoretically possible to do so. In this paper, we propose, design, and implement a new approach to building such a compiler that works with an existing language (P4-16) and an existing hardware architecture (the RMT model).

Our central idea is to employ {\em high-level synthesis} (HLS)~\cite{hls}, taking inspiration from similar approaches to improving designer productivity in FPGAs~\cite{hls_fpga} and digital integrated circuit design~\cite{hls_asic}. Following the lead of prior HLS approaches, we modularize the compilation problem into two pieces: (1) {\em code generation}, which maps a programmer's computations on to the restricted space of transformations supported by a device's computational units, and (2) {\em resource allocation}, which ensures that every program computation and data structure is allocated to some unit within the device. Code generation and resource allocation in our context correspond roughly to the 
scheduling and binding tasks within a traditional HLS workflow (discussed in more detail in \S\ref{ssec:hls}).

Specifically, our modularization of the compilation problem leverages the inherent structure in low-level network packet-processing program representations that use tables with match-action pairs as table entries. We first perform code generation for each \emph{action-computation} in a table, i.e., the P4 program fragment that represents the computation in an action. Note that a table could be part of a user-specified P4 program, or it could be part of a low-level intermediate representation (IR) from a higher level language such as Lyra~\cite{lyra}, Lucid~\cite{lucid}, P4All~\cite{p4all}, etc. Unlike existing compilers, we can handle multi-stage action computations as well as atomic transactions.\footnote{When clear from the context, we will simply say "computation" to refer to a general action-computation.} Our code generation algorithm employs program synthesis to guarantee functional correctness and to efficiently cover the space of semantically-equivalent code that can be mapped to the available computational units in the device. Thus, code generation finds synthesis solutions to ensure that computations can be mapped to available hardware resources based on functionality.

Next, our resource allocation step considers the \emph{global problem over all tables}, to bind the resources needed for each individual computation that have been determined by the earlier code generation step. Here, we take the dependencies between tables into account, such that computations of all tables can be \emph{packed} into available hardware resources (memory, tables, ALUs, etc.) based on capacity. We formulate this as a global constraint problem to find an optimal or a feasible solution, depending on the choice of the user for their program.

Code generation and resource allocation have individually been the focus of prior work~\cite{domino, chipmunk, lavanya_nsdi15, lyra}. One contribution of our work is to combine the two techniques into an overall HLS workflow adapted to the domain of programmable packet processing.
In addition, we present efficient techniques for both code generation and resource allocation. For code generation, we develop an efficient algorithm inspired by digital circuit synthesis, which employs a program synthesis engine, SKETCH~\cite{sketch}, as a subroutine. For resource allocation, we adopt a constraint-based formulation, adapting prior work by Jose et al.~\cite{lavanya_nsdi15} to our setting. This supports finding feasible or optimal solutions by using standard integer-linear programming (ILP) solvers (e.g., Gurobi~\cite{gurobi}) or Satisfiability Modulo Theory (SMT) solvers (e.g., Z3~\cite{z3}).

We prototyped these ideas by designing a compiler, \sysname, that follows an HLS workflow for programmable packet-processing pipelines in the style of RMT. To effectively evaluate \sysname we need a hardware target that supports fine-grained resource allocation and control over the configuration of computation units. Unfortunately, existing commercial switch pipelines have proprietary instruction sets and do not support the kind of low-level access required to prototype \sysname. Hence, we extended Menshen~\cite{menshen_site}, an open-source register-transfer level (RTL) Verilog model of an RMT pipeline, to serve as a hardware target. Because it is written in RTL, this target supports cycle-accurate simulations and can eventually be synthesized into an FPGA or ASIC prototype, although we have not yet performed this synthesis.
%This work does not raise any ethical issues.

%We summarize our contributions below.
%\begin{CompactEnumerate}
%    \item An illustration of the shortcomings of existing commercial compilers for programmable pipelines (\S\ref{sec:motivation}).
%    \item A new approach to building a compiler for programmable switches inspired by high-level synthesis (HLS) (\S\ref{sec:design}).
%    \item Efficient algorithms for code generation and resource allocation within this HLS workflow (\S\ref{ssec:codegen} and \S\ref{ssec:resource_allocation}).
%    \item A prototype compiler, \sysname, that illustrates these ideas by generating machine code for a cycle-accurate simulation of Menshen, along with detailed evaluations (\S\ref{sec:eval}).
%\end{CompactEnumerate}
%We plan to open-source our compiler software along with the benchmarks used in our evaluation.

==> motivation.tex <==
\section{Motivation}
\label{sec:motivation}


We motivate our work using several realistic scenarios showing shortcomings of current compilers for packet-processing pipelines. We list two example scenarios from Cetus~\cite{cetus} and follow this with our own new scenarios. Taken together, they show that there is considerable room for improving compilers.

\Para{Long dependency chains~\cite{cetus}.} A long chain of dependencies between tables in a P4 program can lead to a program requiring more stages than are available in the packet-processing pipeline. This can be remedied by automatically merging pairs of dependent tables into larger tables to shrink inter-table dependency chains.

\Para{Sharing of packet headers~\cite{cetus}.} Variables in a P4 program are mapped onto packet header vector containers; containers are the equivalent of registers in a CPU-based architecture. Naively mapping variables onto containers can exhaust containers, which are a scarce resource. Instead, a smarter compiler can automatically allow variables with  non-overlapping lifetimes to share the same container.

\begin{figure}[t!]
    \centering
    % \vspace{-0.2in}
    \includegraphics[width = \columnwidth]{figures/very_important_ex_small.pdf}
    \vspace{-0.2in}
    \begin{tiny}
    % \caption{Two syntactically different versions of the same P4 program.}
    \caption{Two versions of the same P4 program.}
    \label{fig:motivating_example}
    \end{tiny}
    % \myvspace{-0.15in}
\end{figure}

\begin{figure}[t!]
    \centering
    \vspace{-0.18in}
    \includegraphics[width = \columnwidth,scale=0.5]{figures/Resource_sche.pdf}
    \vspace{-0.2in}
    \begin{tiny}
    % \caption{Resource allocation results from the Tofino compiler for version 1 and version 2.}
     \caption{After compilation, with a limit of 2 tables/stage, version 1 uses more stages than version 2.}
    \label{fig:resource_allo}
    \end{tiny}
    \vspace{-0.13in}
\end{figure}

% \begin{figure}[t!]
%     \centering
%     \vspace{-0.18in}
%     \includegraphics[width = \columnwidth,scale=3.0]{figures/Dependency_graph.pdf}
%     \vspace{-0.2in}
%     \begin{tiny}
%     % \caption{Resource allocation results from the Tofino compiler for version 1 and version 2.}
%      \caption{Dependency graph of benchmark.}
%     \label{fig:dep}
%     \end{tiny}
%     \vspace{-0.13in}
% \end{figure}



\Para{Sub-optimal fitting of programs into pipelines.} Consider a P4 program where the graph of dependencies between tables is sparse. For such a program, the placement of tables into pipeline stages is governed largely by how many tables the pipeline can support per stage. In such cases, we have observed compilers consume more stages than required to map the program onto the underlying hardware. However, reordering statements in the P4 program---where such reordering does not affect program semantics---reduces the stage consumption of the P4 program (Figures~\ref{fig:motivating_example} and ~\ref{fig:resource_allo}).

\Para{Multi-stage actions.} Consider a P4 program with an action consisting of statements that have dependencies between them, i.e., such a program has \emph{intra-action dependencies}, possibly along with \emph{inter-table dependencies}. While such a program is permitted by the P4-16 language specification, it is rejected by the compiler with an error message that indicates that such dependencies are forbidden. However, performing code generation~\cite{hotnets19_codegen, chipmunk} for tables with such actions remedies this issue: a table with intra-action dependencies can be split up into multiple tables in consecutive stages with inter-table dependencies, which can then be mapped onto the hardware. 

\Para{Transaction support.} A more involved example of a multi-stage action is a transactional action that is specified using P4's @atomic annotation~\cite{p4_16_atomic}. An @atomic annotation can be used to surround a block of P4 statements to indicate that they must be executed atomically with respect to the rest of the program. Again, similar to multi-stage actions, while the language specification allows this, compiler support for such transactions is lacking. However, such transactions can again be broken down through code generation into simpler components while ensuring transactional semantics~\cite{domino, chipmunk}; this simplified program can then be mapped to hardware.

\Para{Summary.} As the examples above demonstrate, compilers leave much ``on the table'' in terms of foregoing opportunities for automatic optimization to fit P4 programs into pipelines. Our goal here, taking inspiration from the technique of high-level synthesis~\cite{hls}, is a more systematic approach to the combinatorial problem of resource allocation at the heart of such compilers. To prototype our approach, we target an open-source cycle-accurate simulator of a hardware design~\cite{menshen} coded in RTL Verilog. We do so because we found it extremely challenging to exert low-level control over resource allocation on a proprietary chip such as the Barefoot Tofino~\cite{tofino}. By contrast, with an open-source target, generating machine code is much easier from an engineering perspective since it involves no reverse engineering of an opaque binary.
% -1: keep examples realistic
% 2. Multi-stage actions without atomics (i.e., dependency within an action). Cettus does dependencies between tables---not dependencies betwen actions
% (Table splitting by number of rules is a necessary capability, not a point of departure from Tofino, which already does this in a heuristic manner.)
% Contrast our action-related dependency issue (multi-stage actions) vs. table dependency issue (Cettus' complaint).
% We also do PHV sharing like what Cettus does.

==> old_text/design.tex <==
\iffalse
%% Goals
The main goals for our compiler are to support the following features in P4 programs:
\begin{itemize}
    \item atomic transactions
    \item actions that may need more than one stage -- this is needed for allowing rich actions in atomic transactions and for decomposing tables with wide keys 
    \item multiple atomic transactions.
\end{itemize}
Note that existing compilers have known weaknesses. Specifically, the Tofino compiler does not support any of these features; the Domino and Chipmunk compilers have been shown to work for the first two features, but do not optimize resource allocation for multiple transactions.
%One main goal of our compiler is to support atomic constructs and transaction-style packet-processing programs, where the atomic transactions may get mapped to multiple stages in a hardware pipeline. 
%Following the style supported in the Domino compiler~\cite{domino}, an atomic transaction can be viewed as an action in a match-action table. 
%Since a P4 program contains multiple match-action tables, different atomic transactions will get invoked as actions, depending on the matches that succeed at runtime. Therefore, we consider code generation for each atomic transaction independently of other transactions. 

%% Approach
Our main approach is centered around decomposing the overall problem into: (1) Code generation: for each atomic transaction independently, and (2) Resource allocation: to optimally allocate the available resources to multiple transactions, taking their dependencies into account. 
Note that we perform code generation for a single transaction at a time, which keeps the runtime manageable in practice (as shown in \S\ref{sec:eval}). (These code generation tasks could be parallelized in a future implementation.) As a consequence, the transactions do not share any resources (e.g., stateful updates) -- in future work, we plan to consider static analysis of P4 programs to group together atomic transactions that can potentially share resources.
%, such as for stateful updates. 
\fi %end of commented-out text from earlier version

==> old_text/eval.tex <==
% We also select the commercial compiler like Tofino compiler as another baseline. However, since Tofino compiler does not support atomic P4 actions, comparing the code generation performance will be meaningless (one vs zero comparison). Therefore, we regard Tofino compiler mainly as a resource allocator, which takes one P4-14 program without atomic as an input and allocate several amount of resources for each table to the program runnable in the Tofino switch. And we evaluate the CaT compiler's resource allocation performance by comparing against the Tofino compiler.

% As for resource allocation, we generate P4 programs by selecting some tables from the switch.p4 program and feed them into both Tofino compiler and CaT compiler. Since there is no atomic action in all of the action parts of switch.p4 program, both Tofino and CaT compiler can take them as input and assign each component (e.g., table, action) to corresponding positions. After finding that the heuristic allocation algorithm within the Tofino compiler might lead to suboptimal resource usage result, we move on to generate more P4 programs comprised of tables with artificially defined match-action rules to test how bad it might be if we stick to the Tofino compiler's blackbox allocation algorithm. 

% Finally, as for our own FPGA backend, we generate benchmarks by randomly selecting 2 - 8 tables together with their action blocks from switch.p4  and merge these tables with new tables . 
% There is no existing benchmark compilers to compare against. Therefore, we show the feasibility of the CaT compiler to generate code to different hardware backend by targeting at several FPGA configurations. We also show the benefit of our code generator and the ILP resource allocator.

% by either replacing code generator with some rule-based ones (e.g., Domino compiler) or replacing the ILP code generator by some heuristic ones.

% \Para{Benchmark generation. \xiangyu{Need merging into the main body}}


% \begin{table}[!t]
% \scriptsize
% \centering
% %\begin{tabular}{|p{1.8cm}|p{2.2cm}|p{3.4cm}|}
% \begin{tabular}{||l||l|l||l|l||}
% \hline
% %\textbf{Program} & {\textbf{CaT }} & {\textbf{Tofino compiler (num of stages)}}\\
% \textbf{Program} & \multicolumn{2}{c||}{\textbf{Version 1}} & \multicolumn{2}{c||}{\textbf{Version 2}} \\ 
% \cline{2-5} 
%  & CaT & Tofino & CaT & Tofino\\
% \hline
% Toy Benchmark1 & 12 & reject & 12 & 12 \\
% \hline
% Toy Benchmark2 & 11 & reject & 11 & 11 \\
% \hline
% Toy Benchmark3 & 10 & reject & 10 & 10 \\
% \hline
% Toy Benchmark4 & 9 & reject & 9 & 9 \\
% \hline
% Toy Benchmark5 & 7 & reject & 7 & 7 \\
% \hline
% Real Benchmark1 & 4 & 5 & 4 & 4 \\
% \hline
% Real Benchmark2 & 3 & 4 & 3 & 3 \\
% \hline
% \end{tabular}
% \begin{small}
% \caption{Resource usage by CaT and Tofino compilers.}
% \label{table:Resource usage comparison}
% \end{small}
% \vspace{-0.2in}
% \end{table}

% \begin{table}[!t]
% \scriptsize
% \centering
% %\begin{tabular}{|p{1.8cm}|p{2.2cm}|p{3.4cm}|}
% \begin{tabular}{||l||l|l||l|l||}
% \hline
% \cline{2-5} 
% \textbf{Program} & \textbf{CaT} & \textbf{CaT v1} & \textbf{CaT v2} & \textbf{CaT v3}\\
% \hline
% Benchmark1 & XXX & XXX & XXX & XXX \\
% \hline
% Benchmark2 & XXX & XXX & XXX & XXX \\
% \hline
% Benchmark3 & XXX & XXX & XXX & XXX \\
% \hline
% \end{tabular}
% \begin{small}
% \caption{Resource usage by different versions of CaT.}
% \label{table:Resource usage comparison for CaT}
% \end{small}
% \vspace{-0.2in}
% \end{table}

% \begin{table}[!t]
% \scriptsize
% \centering
% %\begin{tabular}{|p{1.8cm}|p{2.2cm}|p{3.4cm}|}
% \begin{tabular}{||l||l|l||l|l||}
% \hline
% \cline{2-5} 
% \textbf{Program} & \textbf{Configuration 1} & \textbf{Configuration 2} & \textbf{Configuration 3} & \textbf{Configuration 1}\\
% \textbf{Tables/stage} & \textbf{8} & \textbf{7} & \textbf{6} & \textbf{5}\\
% \hline
% Benchmark1 & XXX & XXX & XXX & XXX \\
% \hline
% Benchmark2 & XXX & XXX & XXX & XXX \\
% \hline
% Benchmark3 & XXX & XXX & XXX & XXX \\
% \hline
% \end{tabular}
% \begin{small}
% \caption{TODO: consider some comparisons}
% \label{table:Resource usage comparison for CaT}
% \end{small}
% \vspace{-0.2in}
% \end{table}

% \subsection{Comparing CaT to Tofino}
% We also compare CaT compiler with the existing Tofino compiler to find that there are two major advantages for CaT compiler. On the one hand, it extends the acceptable range of actions within the input P4-16 programs. To be specific, the current Tofino compiler cannot support code generation for P4-16 programs with atomic pragma inside. Even for those programs without atomic pragma, Tofino compiler fails to generate code when there are sequential dependencies within a non-atomic action block. These unnecessarily increase the bar for programmers to write an acceptable P4-16 program because they have to do manual semantically equivalent transformation to turn their programs acceptable by the existing Tofino compiler. However, CaT compiler can deal with these transformations by leveraging a series of code generation tools and optimizing resource allocation algorithms to help programmers avoid worrying too much about these low-level transformation details and focus on program written parts. On the other hand, the optimizing resource allocation algorithm (ILP) baked in the CaT compiler makes its code generation result better than Tofino in terms of the number of stages used. As for several manually generated benchmarks, CaT compiler uses fewer pipeline stages than the Tofino compiler, which likely uses heuristics for resource allocation that do not guarantee the optimal number of stages for every program. This reduction in the number of stages shows the benefit of using an ILP solver rather than heuristics for resource allocation and such a reduction is significant because of the severely constrained number of stages in programmable hardware pipelines. It is easy to generate more benchmarks that CaT compiler can save more than one stage and finally it will lead to a failure vs success result, which means that the Tofino compiler rejects the input program because it overestimated the number of stages required while CaT compiler accepts it. 

==> old_text/intro.tex <==
% Anirudh: continue here...

%\section{Introduction}
\section{Introduction -- Old}
\label{sec:intro}
Programmable packet-processing pipelines are now commercially available both in switches~\cite{tofino} as well as network-interface cards~\cite{pensando}. At the same time, programming these devices continues to be challenging, resulting in numerous proposals for better programming languages for these devices~\cite{lyra, lucid, p4all}. We contend that the problem with programming these devices lies not with the programming language, but rather with the compiler technology under the hood that powers these programming languages. 

A good compiler for any target must have two properties. First, it should be {\em fast}: compile times must be low so as to not bottleneck the programmer. Second, the compiler must generate {\em high quality code} for the target. For programmable packet-processing pipelines, this means the compiler must be able to generate machine code for any program that can fit within the pipeline's limited resources (e.g., memory blocks and arithmetic and logic units (ALUs)). This is important because a program rejected by the compiler cannot run on the underlying target; unlike a processor-based architecture, there is no ``middle ground'' of running a more complicated program at lower performance. When a program is able to fit within the pipeline's resources, it is desirable that the compiler minimizes resource consumption to provide headroom for the program to grow in the future. In trying to meet the dual challenges of fast and high-quality compilation, existing commercial and research compilers for such pipelines face three challenges, detailed below.

\Para{Code Generation.} Programming languages such as P4-16 support the ability to express packet processing as atomic blocks of code~\cite{p4_16_atomic}. In this style, programmers can express packet-processing logic as transactions that manipulate pipeline state and packet headers atomically on every packet. However, despite the availability of such constructs in the P4-16 language, compiler support for such constructs is still rudimentary. Commercial compilers do not yet support it.  Among research compilers, Domino~\cite{domino} supports atomic code generation for such constructs, but often spuriously rejects valid packet-processing programs because the Domino compiler is unable to find a way to map these programs to the underlying instruction set. Chipmunk~\cite{chipmunk} remedies this problem with Domino by making extensive use of program synthesis in the compiler, but its compilation times can be long and highly variable as a result of using synthesis.

\Para{Resource Allocation.} Allocating hardware resources such as memory blocks and ALUs to program constructs such as tables and expressions is a challenging combinatorial problem. Past work has made significant progress on this problem using Integer-Linear Programming (ILP)~\cite{lavanya_nsdi15} and Satisfiability Modulo Theory (SMT) solvers~\cite{lyra}. However, both these projects work with an abstract notion of hardware resources, which do not correspond one-to-one to the actual hardware resources. In more detail, ~\cite{lavanya_nsdi15} works with a very simplified model of the underlying hardware because it was developed before a commercial hardware packet-processing pipeline was available. Lyra~\cite{lyra} achieves resource savings at the level of P4 constructs like registers and tables, but these do not directly correspond to pipeline resources such as memory blocks, ALUs, and stages. Indeed, we have found examples where commercial compilers produce suboptimal resource allocation decisions---likely because they use imperfect heuristics (\S\ref{sec:background}).
 
\Para{Interactions between Code Generation and Resource Allocation.} While code generation and resource allocation are by themselves challenging, their interaction makes the compiler's job even harder. We detail two examples next. First, code generation for a transaction can result in multiple fragments of packet-processing logic with dependencies between them. Each of these fragments must be allocated to an ALU while respecting the hardware's constraints, e.g., on the number of ALUs. Second, opportunities for resource sharing become apparent when code generation and resource allocation interact. For instance, consider a match-action table with a complex action but simple match. This table can be mapped to a pipeline by performing the key lookup for the match in the first pipeline stage. The result from the key lookup is carried to subsequent pipeline stages, where each stage implements a fragment of the action that takes the match result as input. Here the resources for matching are expended only in the first stage and the match process does not need to be repeated in every stage containing an action fragment, freeing those match resources to be used for other tables.

Fundamentally, we believe the compilation problem for packet processing pipelines is challenging because it involves a non-trivial interaction of two distinct combinatorial problems: constrained optimization (e.g., via ILP) for resource allocation, and semantic equivalence/synthesis (e.g., via SMT) for code generation. Theoretical results on the hardness of compilation in the domain of programmable switches~\cite{balazs_hardness} and of code generation for general programs~\cite{AJU77} lend further evidence to this belief.

In response, this paper takes preliminary steps towards building fast {\em optimizing} compilers for packet-processing pipelines. In particular, we introduce a new algorithm for code generation that is better both in terms of the quality of the generated code and code generation time compared with existing approaches. We then introduce an ILP-based approach to resource allocation that builds on ideas introduced by Jose et al.~\cite{lavanya_nsdi15} but instantiates these ideas in the context of real hardware constraints and additionally handles {\em intra-action} dependencies within complex actions as well.

On simple benchmarks, we show that this ILP-based approach produces better resource allocation outcomes than a commercial switch compiler. On a different set of benchmarks, we also show that our new code generation algorithm can produce high-quality code similar to Chipmunk, while providing much fast compilation times than Chipmunk. This work does not raise any ethical issues.
